Streamability of nested word transductions

We consider the problem of evaluating in streaming (i.e., in a single left-to-right pass) a nested word transduction with a limited amount of memory. A transduction T is said to be height bounded memory (HBM) if it can be evaluated with a memory that depends only on the size of T and on the height of the input word. We show that it is decidable in coNPTime for a nested word transduction defined by a visibly pushdown transducer (VPT), if it is HBM. In this case, the required amount of memory may depend exponentially on the height of the word. We exhibit a sufficient, decidable condition for a VPT to be evaluated with a memory that depends quadratically on the height of the word. This condition defines a class of transductions that strictly contains all determinizable VPTs.

==> apx-algorithm.tex <==
\section{Online Evaluation Algorithm of Visibly Pushdown Transductions}%
\label{sec:apx-algo}

All over this section we assume an implementation of \vpts such that
the set $S$ of transitions with a given left-hand side can be
retrieved in time $O(|S|)$.  Recall also that for the presentation of
this algorithm, the \vpt must be reduced.

\subsection{\naive algorithm}
We start with the algorithm \naive,
that we will later improve to obtain \eval.
The algorithm \naive simply computes all the runs
(with their respective outputs)
of the \fvpt $T$ on the input word $u$,
stores them in a data structure
and, at the end of $u$,
outputs the only output word: it will be the same in all accepting runs,
as $T$ is functional.

\naive consists in maintaining the set of \dconfs
corresponding to the runs of $T$ on the input word $u$.
Hence, it is based on the operation $\update(C,a)$ that
returns the set of \dconfs obtained after applying rules
of $T$ using input symbol $a$ to each \dconf of $C$.
The function $\update:\Dconfs T \times \Sigma \to \Dconfs T$
maps a set of \dconfs and an input symbol to another set of \dconfs.
For call symbols $c\in\Sigma_c$,
\begin{displaymath}
\update(C,c) = \bigcup_{(q,\sigma,v)\in C}
\{ (q',\sigma\gamma,vv') \hmid (q,c,v',\gamma,q')\in\delta_c \}
\end{displaymath}
and for return symbols $r\in\Sigma_r$,
\begin{displaymath}
\update(C,r) = \bigcup_{(q,\sigma\gamma,v)\in C}
\{ (q',\sigma,vv') \hmid (q,r,v',\gamma,q')\in\delta_r \}
\end{displaymath}

The function \update can be considered as the transition function
of a transition system with states $\Dconfs T$ (i.e., an infinite number of states).
We can easily turn it into an infinite state transducer,
i.e., an \fst with infinitely many states:
this transducer returns $\epsilon$ at every input symbol,
except for the last one \EOS, where it returns the output word.
This is illustrated in \Figure~\ref{fig:ist-naive}.
\input{figIST-naive}
%
Formally, an infinite state transducer $\istn$ (\ist for short)
is defined exactly like an \fst, except that its number of states
may be infinite (but countable).
In particular, the acceptance condition remains the same,
so that the transduction $\inter \istn$ is still a set of pairs
of finite words $(u,v)$.

Given the functional \vpt $T=(Q,I, F, \Gamma, \delta)$, consider the \ist
$\istn=(\Dconfs T\uplus\{q_f\}, I_\istn, \{q_f\}, \delta_\istn)$
where $I_\istn=\left\{\{(q_0,\bot,\epsilon) \hmid q_0\in I\}\right\}$.
To deal with the last symbol $\EOS$,
we have to characterize the sets of \dconfs reached after
reading words in $\dom(T)$.
$T$ being functional, each of these sets of \dconfs $C$
comes with a single output word $v$:
\[
\mathcal C = \left\{ (C,v)\in\Dconfs T\times\Sigma^* \hmid
\begin{array}{l}
\exists q\in F.\ (q,\bot,v)\in C
\text{ and }\\
\forall (q',\bot,v')\in C,\ q'\in F\implies v'=v
\end{array}
\right\}
\]
Rules in $\delta_\istn$ are:
\[
\begin{array}{ll}
C \xrightarrow{a/\epsilon} \update(C,a) &
\text{ for $C\in\Dconfs T$ and $a\in\Sigma$} \\
C \xrightarrow{\EOS/v} q_f &
\text{ for $(C,v)\in \mathcal C$} \\
\end{array}
\]

\begin{lemma}\label{lem:naive}
$(u,v)\in \inter T$ iff $(u\EOS,v)\in\inter \istn$.
\end{lemma}

\begin{proof}
It can be checked easily by induction on $|u|$
that for every $u\in\Sigma^*$,
the current state of $\istn$ after reading $u$ is
$\bigcup_{q_0\in I}
\{(q,\sigma,v) \hmid (q_0,\bot)\xrightarrow{u/v} (q,\sigma)\}$.
Let us check whether reading the last symbol~\EOS leads to a correct state.
Let $u\in\Sigma^*$.
If $u\notin\dom(T)$, then there is no run of $T$ on $u$ of the form
$(q,\bot)\xrightarrow{u/v}(q',\bot)$ with $q\in I$ and $q'\in F$.
Hence, the state $C$ reached by $\istn$ after reading $u$, if it exists,
is such that $(C,v)\notin\mathcal C$ for all $v\in\Sigma^*$,
so $u\notin\dom(\istn)$.
If $u\in\dom(T)$, then the state of $\istn$ reached after reading $u$
is $C=\bigcup_{q_0\in I}
\{(q,\bot,v) \hmid (q_0,\bot)\xrightarrow{u/v} (q,\bot) \}$.
As $T$ is functional, there is a unique $v$ for all
$(q,\bot,v)\in C$ such that $q\in F$, and such elements of $C$ exist,
so that $(C,v)\in\mathcal C$, and $(u\EOS,v)\in\inter\istn$.
\end{proof}

As $\istn$ is deterministic, the algorithm \naive only consists
in computing the unique run of $\istn$ on the input word $u$.
Let $\maxout(u)=\max_{v\in\reach(u)} |v|$,
and let $\maxoutT(u)$ be its maximal value over prefixes:
$\maxoutT(u)=\max_{u'\text{ prefix of }u}\maxout(u')$.

\begin{proposition}\label{prop:complexity-naive}
The maximal amount of memory used by \naive for processing
$u\in\Sigma^*$ is in
$O(|Q|\cdot|\Gamma|^{h(u)}\cdot\maxoutT(u))$.
The preprocessing time, and the time used by \naive to process each symbol
of $u$ are both polynomial in
$|Q|$, $|\Gamma|$, $|\delta|$, $h(u)$, $\maxoutT(u)$ and $|\Sigma|$.
\end{proposition}

\begin{proof}
  As $T$ is functional, there cannot exist two distinct \dconfs
  $(q,\sigma,v)$ and $(q,\sigma,v')$ that are both accessible and
  co-accessible.
%
  As we suppose that $T$ is reduced, any accessible configuration is co-accessible.
%
  As a consequence, if there are two \dconfs $(q,\sigma,v)$ and
  $(q,\sigma,v')$ in $C$, then we have $v=v'$.
  This remark proves the space complexity.
  %
For time complexity, updating a \dconf is just a research of rules to apply.
Each of them will generate a new \dconf,
and is retrieved in constant time.
\end{proof}



\subsection{Compact representation of runs of \fvpts: \naivecompact.}
%
We present the data structure
$\str{u}{T}$ representing all \dconfs stored by \naive
on the \vpt $T$ after reading $u$, i.e.,
the state of $\istn$ reached after reading $u$.
This structure is illustrated in \Figure~\ref{fig:eval-compact}.
This first improvement avoids the exponential blowup in $h(u)$.
The structure $\str{u}{T}$ is a labeled DAG (directed acyclic graph)
whose nodes are configurations of $T$
(with an additional root node $\rootstr$, and each node has a depth)
and edges are labeled by delays:
$\strnodes{\str{u}{T}} =
\{\rootstr\}\uplus Q\times(\Gamma\cup\{\bot\})\times \Nat$
and
$\stredges{\str{u}{T}} \subseteq
\strnodes{\str{u}{T}}\times\Sigma^*\times\strnodes{\str{u}{T}}$.
This DAG will have as leaves (nodes without outgoing edges)
current configurations.
The structure $\str u T$ is defined inductively on $u$
according to the following algorithms.
\[
\stredges{\str \epsilon T} =
\{ \stredge{\rootstr}{\epsilon}{(q,\bot,0)} \hmid q\in I \}
\]

When a call letter $c\in\Sigma_c$ is read, the structure $\str u T$ is updated
such that, for every leaf of $\str u T$,
a child is added for every way of updating the
corresponding configuration according to a rule of $T$.
If a leaf cannot be updated, it is removed, and also the possible
new generated leaves (procedure \textsc{remove\_edges}).
Algorithm~\ref{algo:update-str-call} describes how $\str {uc} T$ is
computed from $\str u T$.
%
\begin{algorithm}[h]
  \begin{algorithmic}[2]

    \Procedure{update\_call}{$S, c$}
      \State $newEdges \leftarrow \emptyset$
      \State $orphans \leftarrow \emptyset$
      \For {$(q,\gamma,i)\in\strleaves{S}$}
        \If {$\exists v,\gamma',q' \hmid (q,c,v,\gamma',q')\in\delta$}
          \For {$(v,\gamma',q') \hmid (q,c,v,\gamma',q')\in\delta$}
            \State $newEdges.add(\stredge{(q,\gamma, i)}{v}{(q',\gamma',i+1)})$
          \EndFor
        \Else
          \State $orphans.add((q,\gamma,i))$
        \EndIf
      \EndFor
      \State $\stredges{S} \leftarrow \stredges{S} \cup newEdges$
    \EndProcedure
    \State

    \Procedure{remove\_edges}{$S, orphans$}
      \While {$orphans\not=\emptyset$}
        \State $n\leftarrow orphans.pop()$
        \For {$m \hmid \exists v,\ \stredge{m}{v}{n}$}
          \State $remove(S, \stredge{m}{v}{n})$
          \If {$\nexists n',v',\ \stredge{m}{v'}{n'}$}
            $orphans.add(m)$
          \EndIf
        \EndFor
      \EndWhile
    \EndProcedure

  \end{algorithmic}
  \caption{\label{algo:update-str-call} \quad
    Updating structure $S$ with a call symbol.}
\end{algorithm}
%
For a return letter $r\in\Sigma_r$, we try to pop every leaf:
if it is possible, the leaf is removed and the new leaves updated,
otherwise we remove the leaf and propagate the removal upwards
(procedure \textsc{remove\_edges}).
This is described in Algorithm~\ref{algo:update-str-return}.
%
\begin{algorithm}[h]
  \begin{algorithmic}[2]

    \Procedure{update\_return}{$S, r$}
      \State $newEdges \leftarrow \emptyset$
      \State $orphans \leftarrow \emptyset$
      \For {$(q_\ell,\gamma_\ell,i)\in\strleaves{S}$}
        \If {$\exists v,q \hmid (q_\ell,r,v,\gamma_\ell,q)\in\delta$}
          \For {$(v,q) \hmid (q_\ell,r,v,\gamma_\ell,q)\in\delta$}
            \For {$(q_0,\gamma_0,v_0) \hmid
              \stredge{(q_0,\gamma_0,i-1)}{v_0}{(q_\ell,\gamma_\ell,i)}
              \in\stredges{S}$}
              \For {$(n,v_1) \hmid
                \stredge{n}{v_1}{(q_0,\gamma_0,i-1)}
                \in\stredges{S}$}
                \State $newEdges.add(\stredge{n}{v_1v_0v}{(q,\gamma_0,i-1)})$
              \EndFor
            \EndFor
          \EndFor
        \Else
          \State $orphans.add((q_\ell,\gamma_\ell,i))$
        \EndIf
      \EndFor
      \State $remove\_edges(S, orphans)$
      \State $remove\_leaves(S)$
      \State $\stredges{S} \leftarrow \stredges{S} \cup newEdges$
    \EndProcedure
    \State

    \Procedure{remove\_leaves}{$S$}
      \For {$n\in\strleaves{S}$}
        \For {$(m,v) \hmid \stredge{m}{v}{n} \in \stredges{S}$}
          \State $remove(S, \stredge{m}{v}{n})$
        \EndFor
      \EndFor
    \EndProcedure
  \end{algorithmic}
  \caption{\label{algo:update-str-return} \quad
    Updating structure $S$ with a return symbol.}
\end{algorithm}
%
Only edges and reachable nodes need to be stored, so that
$|\str u T| \le (\hc(u)+1)\cdot|Q|^2\cdot|\Gamma|^2\cdot\maxout(u,T)$.

We prove the correctness of this construction using
the transition function $\stredgeSem{u}{}{}{}$
based on edges of $\str u T$,
that gathers the stack content and delay.
The relation $\stredgeSem{u}{}{}{}$ is the smallest relation
in $(Q\times\Gamma^*\times\Nat)\times\Sigma^*\times(Q\times\Gamma^*\times\Nat)$
containing $\stredge{}{}{}$ such that:
if $\stredgeSem{u}{(q_0,\sigma_0,i)}{v}{(q_1,\sigma_1\gamma,j)}$
and $\stredge{(q_1,\gamma,j)}{v'}{(q_2,\gamma',j+1)}$
then $\stredgeSem{u}{(q_0,\sigma_0,i)}{vv'}{(q_2,\sigma_1\gamma\gamma',j+1)}$
(we may have $\sigma=\emptyword$ and $\gamma=\bot$).
The set of \dconfs stored in $\str u T$ is defined by:
$\strSem{\str u T} = \{ (q,\sigma,v) \hmid
\exists i,\ (q,\sigma,i)\in\strleaves{\str u T}\text{ and }
\stredgeSem{u}{\rootstr}{v}{(q,\sigma,i)}\}$.
The following lemma shows that $\str u T$ exactly encodes
the \dconfs computed by the \ist $\istn$.

\begin{lemma}\label{lem:correctness-str}
$\strSem{\str u T}$ is the state of the \ist $\istn$ after reading $u$.
\end{lemma}

\begin{proof}
As mentioned in the proof of Lemma~\ref{lem:naive},
the current state of $\istn$ after reading $u$ is
$\bigcup_{q_i\in I}
\{(q,\sigma,v) \hmid (q_i,\bot)\xrightarrow{u/v} (q,\sigma)\}$.
Hence proving the following invariant is sufficient to prove this lemma:
\begin{quote}
For every $0\le i\le \hc(u)$,
$\stredgeSem{u}{\rootstr}{v}{(q,\sigma,i)}$ iff
there exists $q_i\in I$ such that
$(q_i,\bot)\xrightarrow{u_1\cdots u_k/v}{(q,\sigma)}$
where $k=\max \{j \hmid \hc(u_1\cdots u_j) = i\}$.
\end{quote}
We prove it by induction on $|u|$.
%
If $|u|=0$, then $i=0$ and the equivalence holds,
as we can assume $\emptyword$-loops (without output) on initial states.

Assume that the property holds for a given $u$,
we prove that if also holds for the well-nested prefix $uc$.
Let $orphans$ be the set of leaves collected by the outermost
for-loop of \textsc{update\_call}.
These are the leaves $(q,\gamma,\hc(u))$ of $\str u T$ such that no rule
$(q,c,v,\gamma',q')$ exists in $\delta$.
Hence, corresponding configurations are blocked, and can be removed.
The procedure \textsc{remove\_edges} propagates these deletions,
so that after the call to this procedure, the structure
exactly contains configurations that can be updated by $c$.
%
Hence, by induction hypothesis, the equivalence holds for $0\le i\le \hc(u)$.
For $i=\hc(uc)=\hc(u)+1$,
let $k=\max \{j \hmid \hc(u_1\cdots u_j) = i\}$.
We have:
\[
\begin{array}{lc}
\stredgeSem{uc}{\rootstr}{vv'}{(q,\sigma\gamma\gamma',i)} & \\
\quad \text{iff}\quad
\exists q_1,\ \stredgeSem{uc}{\rootstr}{v}{(q_1,\sigma\gamma,i-1)}
\quad\text{ and }\quad
\stredge{(q_1,\gamma,i-1)}{v'}{(q,\gamma',i)}
& (1) \\
\quad \text{iff}\quad
\exists q_1,\ \exists q_i\in I,\ (q_i,\bot)\xrightarrow{u/v}{(q_1,\sigma\gamma)}
\quad\text{ and }\quad
\stredge{(q_1,\gamma,i-1)}{v'}{(q,\gamma',i)}
& (2) \\
\quad \text{iff}\quad
\exists q_1,\ \exists q_i\in I,\ (q_i,\bot)\xrightarrow{u/v}{(q_1,\sigma\gamma)}
\quad\text{ and }\quad
(q_1,c,v',\gamma',q)\in\delta
& (3) \\
\quad \text{iff}\quad
\exists q_i\in I,\ (q_i,\bot)\xrightarrow{uc/vv'}{(q,\sigma\gamma\gamma')}
& \\
\end{array}
\]
$(1)$ is by definition of $\stredgeSem{uc}{}{}{}$.
$(2)$ holds because, as mentioned above,
\textsc{remove\_edges} removes non-accessible configurations,
and by induction hypothesis.
Here, we also have $k-1=\max \{j \hmid \hc(u_1\cdots u_j) = i-1\}$, as
$uc$ ends with a call symbol: so $u_1\cdots u_{k-1}=u$ and
$u_1\cdots u_k=uc$.
$(3)$ is due to the way \textsc{update\_call} operates:
it adds children to leaves according to rules of $\delta$.

Now we show that the property holds for the well-nested prefix $ur$,
if it holds for $u$.
Let $h=\hc(u)$.
Procedure \textsc{update\_return} checks, for each leaf, whether a rule
can be applied. If not, the leaf is removed, and orphaned edges too,
as explained for call symbols.
Then, the $h$th level is removed and the $(h-1)$th updated, according to rules
of $T$.
Hence the property remains true for $0\le i\le h-2$.
We have:
\[
\begin{array}{lc}
\stredgeSem{ur}{\rootstr}{v}{(q,\sigma\gamma\gamma_0,h-1)} & \\
\quad \text{iff}\quad
\exists q_0,q_1,q_\ell,\gamma_\ell,v',v_0,v_1,\
\stredgeSem{u}{\rootstr}{v'}{(q_1,\sigma\gamma,h-2)}\text{ and }\\
\qquad\qquad
\stredge{(q_1,\gamma,h-2)}{v_1}{(q_0,\gamma_0,h-1)}\in\stredges{\str u T}
\text{ and }\\
\qquad\qquad
\stredge{(q_0,\gamma_0,h-1)}{v_0}{(q_\ell,\gamma_\ell,h)}\in\stredges{\str u T}
\text{ and }\\
\qquad\qquad
(q_\ell,r,v'',\gamma_\ell,q)\in\delta\text{ and }
v=v'v_1 v_0 v''
& (1) \\
\quad \text{iff}\quad
\exists q_0,q_\ell,\gamma_\ell,v',v_0,\
\stredgeSem{u}{\rootstr}{v'}{(q_0,\sigma\gamma\gamma_0,h-1)}
\text{ and }\\
\qquad\qquad
\stredge{(q_0,\gamma_0,h-1)}{v_0}{(q_\ell,\gamma_\ell,h)}\in\stredges{\str u T}
\text{ and }\\
\qquad\qquad
(q_\ell,r,v'',\gamma_\ell,q)\in\delta\text{ and }
v=v' v_0 v''
& (2) \\
\quad \text{iff}\quad
\exists q_\ell,\gamma_\ell,v',\
\stredgeSem{u}{\rootstr}{v'}{(q_\ell,\sigma\gamma\gamma_0\gamma_\ell,h)}\in\stredges{\str u T}
\text{ and }\\
\qquad\qquad
(q_\ell,r,v'',\gamma_\ell,q)\in\delta\text{ and }
v=v'v''
& (3) \\
\quad \text{iff}\quad
\exists q_\ell,\gamma_\ell,v',q_i\in I\
(q_i,\bot)\xrightarrow{u/v'}{(q_\ell,\sigma\gamma\gamma_0\gamma_\ell)}
\text{ and }\\
\qquad\qquad
(q_\ell,r,v'',\gamma_\ell,q)\in\delta\text{ and }
v=v'v''
& (4) \\
\quad \text{iff}\quad
\exists q_i\in I,\ (q_i,\bot)\xrightarrow{ur/v}{(q,\sigma\gamma\gamma_0)}
& \\
\end{array}
\]
Equivalence $(1)$ reflects how \textsc{update\_return} generates the
new leaves.
$(2)$ and $(3)$ come from the definition of $\stredgeSem{u}{}{}{}$.
$(4)$ is obtained by induction hypothesis and the fact that,
if $k=\max \{j \hmid \hc(u_1\cdots u_j) = h\}$, then
$u_1\cdots u_k=u$.
\end{proof}

The depth of the DAG obtained after reading $u$ is
the current height of $u$ plus~$1$,
each level has at most $|Q|\cdot|\Gamma|$ nodes,
and each edge is labelled with a word of length less than
$\maxout(u)$.

\begin{proposition}\label{prop:complexity-naive-compact}
The maximal amount of memory used by \naivecompact on $u\in\Sigma^*$ is in
$O(|Q|^2\cdot|\Gamma|^2\cdot (h(u)+1)\cdot\maxoutT(u))$.
The preprocessing time, and the time used by \naive to process each symbol
of $u$ are both polynomial in
$|Q|$, $|\Gamma|$, $|\delta|$, $h(u)$, $\maxoutT(u)$ and $|\Sigma|$.
\end{proposition}


\subsection{\eval algorithm}

We extend the definition of the largest common prefix to sets of \dconfs:
if $C\subseteq\Dconfs T$, then
$\lcp C = \lcp {\{v \hmid (q,\sigma,v)\in C\}}$.
Let \remlcp be the function that removes the largest common prefix
to a set of \dconfs:
$
\remlcp(C) = \{ (q,\sigma,v')\in\Dconfs T \hmid
(q,\sigma,\lcp C \cdot v')\in C\}
$.
%
From an \fvpt $T$, we define
the \ist $\iste=(\Dconfs T\uplus\{q_f\},I_\iste,\{q_f\},\delta_\iste)$
where $I_\iste=\{\{(q_0,\bot,\epsilon) \hmid q_0\in I\}\}$.
We keep the same definition of $\mathcal C$ as in \naive,
and rules of $\delta_\iste$ are:
\[
\begin{array}{ll}
C \xrightarrow{a/\lcp{\update(C,a)}} \remlcp(\update(C,a)) &
\text{ for $C\in\Dconfs T$ and $a\in\Sigma$} \\
C \xrightarrow{\EOS/v} q_f &
\text{ for $(C,v)\in \mathcal C$} \\
\end{array}
\]
We start by proving the correctness of the definition of the \ist $\iste$.
This definition is illustrated in \Figure~\ref{fig:ist-eval}.
\input{figVPT}
\input{figIST-eval}

\begin{lemma}\label{lem:eval}
$(u,v)\in \inter T$ iff $(u\EOS,v)\in\inter \iste$.
\end{lemma}

\begin{proof}
By an induction on $|u|$, it can be checked that
$C_0\xrightarrow{u/\lcpin u T}_\iste C$
where $C_0$ is the only element in $I_\iste$
and $C$ is obtained from the run of $\istn$ on $u$:
$C=\remlcp(C')$ with $C_0\xrightarrow{u/\epsilon}_\istn C'$.
The remainder of the proof is similar to the proof of Lemma~\ref{lem:naive}.
\end{proof}

We now provide algorithms for the second step of
the computation performed by \eval on an input symbol $a$.
Recall that the first step is the same as in \naivecompact,
i.e. Algorithm~\ref{algo:update-str-call} if $a$ is a call symbol, and
Algorithm~\ref{algo:update-str-return} if it is a return symbol,
which transforms $\str u T$ to a new structure $S'$.
The second step is the computation of $\lcp{\strSem{S'}}$, which is output,
and removed from every branch of $S'$, using Algorithm~\ref{algo:lcp}.

Algorithm~\ref{algo:lcp} starts with the procedure \factorize,
that processes every nodes in a bottom-up manner
(from leaves to the root \rootstr).
For every node, the lcp of all outgoing edges is moved to all incoming edges.
This is illustrated in \Figure~\ref{fig:factorize}.

\begin{figure}%[!ht]
\centering
\subfloat[Internal node $n$ of the DAG.]{
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,semithick]
\node (n) {$n$};
\node (i1) [above left =1cm and 1cm of n] {};
\node (i2) [above right=1cm and 1cm of n] {};
\node (o1) [below left =1cm and 1cm of n] {};
\node (o2) [below=1.1cm of n]             {};
\node (o3) [below right=1cm and 1cm of n] {};
\draw (i1) -- node                     {$a$}   (n);
\draw (i2) -- node [above,xshift=-1mm] {$b$}   (n);
\draw (n)  -- node [above,xshift=-2mm] {$abc$} (o1);
\draw (n)  -- node [pos=.6]            {$aba$} (o2);
\draw (n)  -- node [above,xshift=2mm]  {$aba$} (o3);
\end{tikzpicture}} % chktex 31
%
\hspace{2cm}
%
\subfloat[Node $n$ after update by \factorize.]{
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,semithick]
\node (n) {$n$};
\node (i1) [above left =1cm and 1cm of n] {};
\node (i2) [above right=1cm and 1cm of n] {};
\node (o1) [below left =1cm and 1cm of n] {};
\node (o2) [below=1.1cm of n]             {};
\node (o3) [below right=1cm and 1cm of n] {};
\draw (i1) -- node                     {$aab$}   (n);
\draw (i2) -- node [above,xshift=-2mm] {$bab$}   (n);
\draw (n)  -- node [above,xshift=-2mm] {$c$} (o1);
\draw (n)  -- node [pos=.6]            {$a$} (o2);
\draw (n)  -- node [above,xshift=2mm]  {$a$} (o3);
\end{tikzpicture}} % chktex 31
%
\caption{Changes performed by \factorize on a node.}\label{fig:factorize}
\vspace{-4mm}
\end{figure}

\begin{algorithm}[h]
  \begin{algorithmic}[2]

    \Procedure{output\_lcp}{$S$}
      \State $factorize(S, \rootstr, \emptyset)$
      \State $\ell \leftarrow \lcp{\{ v \hmid \exists n,\ \stredge{\rootstr}{v}{n}\}}$
      \State \textbf{output} $\ell$
      \For {$m,v \hmid \stredge{\rootstr}{v}{m}$}
        \State let $p$ be such that $v=\ell\cdot p$
        \State replace $\stredge{\rootstr}{v}{m}$ by $\stredge{\rootstr}{p}{m}$ in $S$
      \EndFor
    \EndProcedure
    \State

    \Function{factorize}{$S$, $n$, $done$}
      \If {$n\notin\strleaves{S}$}
      \For {$m,v \hmid \stredge{n}{v}{m}$ and $m\notin done$}
        \State $done\leftarrow factorize(S, m, done)$
      \EndFor
      \If {$n=\rootstr$}
        \Return $done\cup\{n\}$
      \EndIf
      \State $factor\leftarrow\lcp{\{ v \hmid \exists m,\ \stredge{n}{v}{m}\}}$
      \For {$m,v \hmid \stredge{n}{v}{m}$}
        \State let $p$ be such that $v=factor\cdot p$
        \State replace $\stredge{n}{v}{m}$ by $\stredge{n}{p}{m}$ in $S$
      \EndFor
      \For {$p,v \hmid \stredge{p}{v}{n}$}
        \State replace $\stredge{p}{v}{n}$ by $\stredge{p}{v\cdot factor}{n}$ in $S$
      \EndFor
      \EndIf
      \State \Return $done\cup\{n\}$
    \EndFunction

  \end{algorithmic}
  \caption{\label{algo:lcp} \quad
    Compute $\lcp{\strSem S}$, and update $S$ to the structure encoding $\remlcp(\strSem S)$.}
\end{algorithm}

For every node $n\in\strnodes{\str u T}$,
let $S_n$ be the structure obtained from $\str u T$ just after
returning from $\factorize(S, n, done)$, and
let $\stredgeSem{n}{}{}{}$ be the relation defined like $\stredgeSem{u}{}{}{}$,
but on $S_n$.
Note that the structure has the same set of nodes and edges
after being processed by Algorithm~\ref{algo:lcp},
only the labels of edges are updated.
Let $B_n$ be the set of branches from node $n$ to a leaf:
$B_{n_0} = \{(n_0,n_1,\dots,n_k) \hmid \forall 0\le i<k,\ \exists v_i,\
\stredge{n_i}{v_i}{n_{i+1}} \text{ and } n_k\in\strleaves{\str u T}\}$.
For a branch $b$, we write $V_n(b)$ for its output in the structure $S_n$,
and $V(b)$ for its output in $\str u T$:
$V_n((n_0,\dots,n_k))=v_0\cdots v_{k-1}$ where
$\stredge{n_i}{v_i}{n_{i+1}}$ for all $0\le i< k$ in $S_n$.
We extend this definition to sets of branches:
$V_n(B) = \{V_n(b)\hmid b\in B\}$.
Note also that each node is processed once using \factorize,
and in a bottom-up way: when processing node $n$,
all its descendants have been updated before (cf lines 11 and 12).
The following property is the main invariant proving the correctness of
Algorithm~\ref{algo:lcp}.

\begin{lemma}\label{lem:factorize}
For every node $n\not=\rootstr$,
let $\ell = \lcp{V(B_n)}$.
Then,
\begin{enumerate}
\item for every branch $b\in B_n$, $V(b) = \ell\cdot V_n(b)$
\item for every $p,v$ such that $\stredge{p}{v}{n}$ in $S_n$,
$v = v'\ell$ with $\stredge{p}{v'}{n}$ in $\str u T$
\end{enumerate}
\end{lemma}

\begin{proof}
We prove the following property by bottom-up induction on the structure.
This property is true on leaves, as \factorize does not modify their
incoming edges.
Assume that the property holds for all descendants of a node $n$.
Let $\ell = \lcp{V(B_n)}$, and consider a branch $b\in B_n$.
The function \factorize applied at $n$ computes the lcp of edges
outgoing from $n$ and removes it on every branch.
Hence, if $n'$ be the node processed by \factorize before $n$,
then:
\begin{equation} \label{eqn:factorize1}
V_{n'}(b) =
\lcp{\{v\hmid \exists p,\ \stredge{n}{v}{p}\text{ in } S_{n'}\}}\cdot V_n(b)
\end{equation}
Let $p$ be the second node in branch $b=(n,p,\ldots)$.
As $p$ and all its descendants are processed before $n'$ and
not modified until the call of \factorize on $p$, we have
$V_{n'}(b)=V_p(b)$.
Let us decompose $V_p(b)$ according to $p$:
$V_p(b)=v_0\cdot V_p(b_p)$ where $\stredge{n}{v_0}{p}$ in $S_p$ and
$b_p$ is the branch obtained from $b$ by removing $n$.
Using the induction hypothesis applied at $p$, we get
$v_0=v_1\ell'$ with $\ell'=\lcp{V(B_p)}$,
$\stredge{n}{v_1}{p}$ in $\str u T$,
and $V(b_p)=\ell'\cdot V_p(b_p)$.
Thus $V_p(b)=v_1\cdot\ell'\cdot V_p(b_p)=v_1\cdot V(b_p)=V(b)$.
Equation~(\ref{eqn:factorize1}) becomes:
%
\begin{equation} \label{eqn:factorize2}
V(b) =
\lcp{\{v\hmid \exists p,\ \stredge{n}{v}{p}\text{ in } S_{n'}\}}\cdot V_n(b)
\end{equation}
Let us write $\ell''=
\lcp{\{v\hmid \exists p,\ \stredge{n}{v}{p}\text{ in } S_{n'}\}}$.
It remains to prove that $\ell''=\ell$.
Notice that this will prove both parts of the lemma.
We have
$\ell''=\lcp{\{v\hmid \exists p,\ \stredge{n}{v}{p}\text{ in } S_{p}\}}$
because $p$ and its descendants are unchanged between calls of
\factorize on $p$ and $n'$.
Using the induction hypothesis on each $p$, we obtain:
\[
\ell''=
\lcp{\{v\cdot\lcp{V(B_p)}
\hmid\stredge{n}{v}{p}\text{ in } \str u T\}}
=\lcp{V(B_n)}
=\ell
\]
This concludes the proof.
\end{proof}

\ignore{
Let $F(\str u T)$ be the structure obtained after
applying function \factorize of Algorithm~\ref{algo:lcp} to $\str u T$.
The following lemma shows that the lcp of branches below a node is empty.

\begin{lemma}
For every node $n\in\strnodes{F(\str u T)}$ different from $\rootstr$,
\[
\lcp{\{v\hmid \exists m\in\strleaves{F(\str u T)},\
\stredgeSem{}{n}{v}{m}\}}=\emptyword
\]
\end{lemma}

\begin{proof}
Nodes are unchanged once processed,
so $\lcp{\{v\hmid \exists m\in\strleaves{F(\str u T)},\
\stredgeSem{}{n}{v}{m}\}}=\lcp{V_n(B_n)}$ for every node $n\not=\emptyset$.
\[
\begin{array}{lll}
\lcp{V(B_n)} & = \lcp{\{V(b) \hmid b\in B_n\}} \\
& = \lcp{\{\lcp{V(B_n)}\cdot V_n(b) \hmid b\in B_n\}}
& \text{ by Lemma~\ref{lem:factorize}}\\
& = \lcp{V(B_n)}\cdot \lcp{\{V_n(b) \hmid b\in B_n\}} & \\
& = \lcp{V(B_n)}\cdot \lcp{V_n(B_n)} & \\
\end{array}
\]
So $\lcp{V_n(B_n)}=\emptyset$.
\end{proof}
}

The next lemma ensures that \factorize preserves the semantic
of the structure, i.e., the set of encoded configurations.

\begin{lemma}\label{lem:factorize-sem}
$\strSem{F(\str u T)}=\strSem{\str u T}$.
\end{lemma}

\begin{proof}
\[
\begin{array}{ll}
(q,\sigma,v)\in\strSem{\str u T} \\
\qquad \text{ iff }
\exists i,\ (q,\sigma,i)\in\strleaves{\str u T}\text{ and }
\stredgeSem{u}{\rootstr}{v}{(q,\sigma,i)} \\
\qquad \text{ iff }
\exists i,\ (q,\sigma,i)\in\strleaves{\str u T}\text{ and }
\exists p,\ \stredge{\rootstr}{v_0}{p}\text{ and }
\stredgeSem{u}{p}{v_1}{(q,\sigma,i)}
\text{ with } v = v_0v_1 \\
\qquad \text{ iff }
\exists i,\ (q,\sigma,i)\in\strleaves{\str u T}\text{ and }
\exists p,\ \stredge{\rootstr}{v_0}{p}\text{ and }
v = v_0V(b) \\
\qquad\qquad
\text{ where $b$ is a branch $\stredgeSem{u}{p}{}{(q,\sigma,i)}$}\\
\qquad \text{ iff }
\exists i,\ (q,\sigma,i)\in\strleaves{\str u T}\text{ and }
\exists p,\ \stredge{\rootstr}{v_0}{p}\text{ and }
v = v_0\cdot\lcp{V(B_p)}\cdot V_n(b) \\
\qquad\qquad
\text{ where $b$ is a branch $\stredgeSem{u}{p}{}{(q,\sigma,i)}$} &
(1)\\
\qquad \text{ iff }
(q,\sigma,v)\in\strSem{F(\str u T)} \\
\end{array}
\]
Equivalence $(1)$ is by Lemma~\ref{lem:factorize}.
\end{proof}

\begin{proof}[Proposition~\ref{prop:complexity-eval}]
  Let us first show that given a reduced \fvpt $T$,
  Algorithm \eval runs, on an input word $u$, in space
  complexity $O(|Q|^2\cdot|\Gamma|^2\cdot
  (h(u)+1)\cdot\maxoutdiffT(u))$.
%
Correctness of Algorithm~\ref{algo:lcp}
is ensured by Lemma~\ref{lem:factorize},
and the fact that at the root node,
it uses the same technique to factorize and output the lcp.
In terms of memory requirement,
the number of nodes of $\str u T$ remains bounded as before,
while words on edges have length at most $\maxoutdiffT(u)$,
as each of them participate in a \dconf in $\strSem{\str u T}$,
as proved by Lemma~\ref{lem:factorize-sem} and Lemma~\ref{lem:correctness-str}.

\medskip Consider now an arbitrary \fvpt $T$. If $T$ is not reduced,
then we reduce it in polynomial time. Then, we can consider the Turing
Transducer associated with algorithm \eval. It can be constructed in
polynomial time, by correction of Algorithm \eval it computes the
transduction $\inter{T}$, and by the above property of Algorithm
\eval, it runs in space complexity $O((h(u)+1)\cdot\maxoutdiffT(u))$.
%All procedures are in polynomial time.
\end{proof}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> apx-streaming.tex <==
\section{Bounded Memory Evaluation Problems}%
\label{apx:BM}

\subsection{Bounded Memory functional \fsts}
%Proof of Proposition~\ref{prop:bmfst}, statements 1 and 2}

\begin{proposition}\label{prop:bmfst}\label{prop:bmpt}
  Let $T$ be a functional \fst.
\begin{enumerate}
 %\noindent \textbf{1.}
  \item $\inter{T}$ is BM iff $T$ is sequentializable;
 %\textbf{2.}
  \item It is decidable in \ptime if $\inter{T}$ is BM~\cite{DBLP:journals/iandc/WeberK95}.
%  \item Bounded memory is undecidable for pushdown transducers.
\end{enumerate}
\end{proposition}

% TEMP
\begin{proof}
  Statement 2 is proved in~\cite{DBLP:journals/iandc/WeberK95} (it is proved that
  sequentializability is decidable in \ptime). We prove statement 1.
  Clearly, if $\inter{T}$ is definable by a sequential transducer
  $T_d$, then evaluating $T_d$ on any input word $u$ can be done with
  a space complexity that depends on the size of $T_d$ only.


  Conversely, if $\inter{T}$ is BM, there exists $K\in\Nat$ and a TT
  $M$ that transforms any input word $u$ into $\inter{T}(u)$ in space
  complexity $K$. Any word on the working tape of $M$ is of length at
  most $K$. As $M$ is deterministic, we can therefore see $M$ as a
  sequential \fst, whose states are pairs $(q,w)$ where $q$ is a
  state of $T$ and $w$ a word on the working tape (modulo some
  elimination of $\epsilon$-transitions).


%%   \fst\ms{Manu: on va un peu vite, la transformation n'est pas
%%     immediate, car on peut avoir des transitions epsilon qui
%%     produisent des mots (mais pas de boucles), du coup
%%     on peut tout tasser a droite, et de plus sur les machines de Turing il y a
%%     toujours un symbole de fin. Ca vaudrait le coup de bien ecrire ca
%%     en appendix, en etant plus formel pour le model}


%% We can see $M$ as an FST $T_M$ with $\epsilon$-transitions which can
%% also produce outputs: the states of $T_M$ are configurations of the
%% machine (there are boundedly many as $M$ uses a space $K$).


%% If from a configuration $c$ $M$ reads an input letter $a\in\Sigma$ and goes to
%% a configuration $c'$, we add the transition $c\xrightarrow{a|\epsilon} c'$ to
%% $T_M$.


%% If from a configuration $c$ $M$ writes a letter $a\in\Sigma$ on the output tape and goes to
%% a configuration $c'$, we add the transition $c\xrightarrow{\epsilon|a}
%% c'$.


%% If from a configuration $c$ $M$ does something on the working tape and
%% goes to the configuration $c'$ in one step, we add the transition
%% $c\xrightarrow{\epsilon|\epsilon} c'$.


%% It might also be the case that $M$ reads a blank symbol $\perp$ on the input
%% tape, in this case we create the transition of $T_M$ as for symbols of
%% $\Sigma$.


%% We have now to turn $T_M$ as a subsequential transducer $T$. First we
%% eliminate transitions $c\xrightarrow{\epsilon|\epsilon} c'$ with
%% classical techniques of automata theory.


%% For transitions of the form $c\xrightarrow{\epsilon|w} c'$ where
%% $w\neq\epsilon$, there cannot be cycles which contains such kind
%% of transitions (otherwise the computation would not terminate).
%% Therefore we can push the words $w$ to the right up to
%% the first non-epsilon transition, if it exists. \ms{Manu:explain what
%%   happens if it does not exist)}.
%% Then we again remove
%% transitions of the form $c\xrightarrow{\epsilon|\epsilon} c'$.


%% Sequentiality is given by all the output words produces after
%% reading the first blank symbol on the input tape.

%% Accepting states are configurations of $M$ which are in an accepting
%% state.
\end{proof}


\subsection{Bounded Memory pushdown transductions}
%Proof of Proposition~\ref{prop:bmpt}, statement 3}

\begin{proposition}
  It is undecidable whether a pushdown transduction is BM\@.
\end{proposition}

\begin{proof}
  We reduce the problem of deciding whether the language of a pushdown
  automaton $P$ over an alphabet $A$ is regular to BM\@. Any letter of $A$ is
  seen as an internal symbol.  We associate
  with $P$ a pushdown transducer $I_P$ which defines the identity on $L(P)$.
  Clearly, if $L(P)$ is regular, it is defined by a finite automaton which can
  easily be turned into a Turing transducer defining $\inter{I_P}$ and
  which uses a memory that depends on the size of the automaton only.
  Conversely, if $\inter{I_P}$ is BM, there exists a function $f$ and
  a TT $M$ equivalent to $I_P$ and which uses at most $f(1,|M|)$ bits
  of memory, i.e., an amount of memory which depends on the size of $M$
  only. The machine $M$ can easily be turned into a finite automaton
  which defines $P$, whose states are the configurations of the
  working tape of $M$.
\end{proof}


\subsection{Proof of Proposition~\ref{thm:bmvpts}}

\begin{proof}
  If $\inter{T}$ is BM, there exist $K$ and a TT $M$ such that $M$
  evaluates any input word in space at most $K$. We can easily extract
  from $M$ a finite automaton that defines $\dom(T)$, whose number of
  states $m$ only depends on $M$ and $K$. By a simple pumping
  argument, it is easy to show that the words in $\dom(T)$ have a
  height bounded by $m$. If the height of the words in $\dom(T)$ is
  bounded, then their height is bounded by $n^2$. Indeed, assume that
  there exists a word $u\in\dom(T)$ whose height is strictly larger
  than $n^2$. Then there exists a run of $T$ on $u$ of the following
  form:
  \[
  (i,\bot) \xrightarrow{u_1/v_1} (q,\sigma) \xrightarrow{u_2/v_2}
  (q,\sigma\sigma') \xrightarrow{u_3/v_3} (p,\sigma\sigma')
  \xrightarrow{u_4/v_4} (p,\sigma) \xrightarrow{u_5/v_5} (f,\bot)
  \]
  such that $u=u_1u_2u_3u_4u_5$, $\sigma'$ is not empty, and $i$
  (resp. $f$) is an initial (resp.\ final) state of $T$. The existence
  of this decomposition follows from the consideration of the set of
  pairs of positions in $u$ corresponding to matching calls and
  returns of well-nested subwords of $u$. Then one can iterate the
  matching loops around $q$ and $p$ to generate words in $\dom(T)$
  with arbitrarily large heights, yielding a contradiction.
%  it is also easy to show by a pumping technique on the
%  $\vpt$ that it is bounded by $n^2$ (otherwise we can find two
%  ``well-nested'' loops, which can be pumped in parallel to increase the height
%  unboundedly\ms{manu:explain more}.
  Therefore $\fst(T,n^2)$ is equivalent to $T$. As in the proof of
  Proposition~\ref{prop:bmfst}, we can regard $M$ as a sequential \fst
  $T_M$ whose set of states are configurations of the machine. The
  \fst $T_M$ is equivalent to $T$, and therefore to
  $\fst(T,n^2)$. Since $T_M$ is sequential, $\fst(T,n^2)$ is
  sequentializable and therefore by Proposition~\ref{prop:bmfst},
  $\fst(T,n^2)$ is BM\@. The converse is obvious.


  Therefore to check whether $\inter{T}$ is BM, we first decide if the height of all input words
  accepted by $T$ is less or equal than $n^2$. This can be done in
  \ptime $O(|T|\cdot n^2)$ by checking emptiness of the projection of
  $T$ on the inputs (this is a visibly pushdown automaton) extended
  with counters up to $n^2+1$ that counts the height of the word.
  Then we check in \conptime whether evaluating $T$ can be done in
  constant memory if we fix both the transducer and the height of the
  word (Theorem~\ref{thm:vptsboundedmem}). Since here the
  height is bounded by $n^2$, it is equivalent to checking bounded
  memory.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> apx-twinning.tex <==
\section{On deciding height bounded memory for \vpts}

Before going into the proofs of the results of this section, we first
prove that our horizontal twinning property, when restricted to
\fsts, is equivalent to the twinning property for \fsts defined
in~\cite{DBLP:journals/tcs/BealC02}.


\subsection{Twinning properties for \fsts}%
\label{apx:equiv-twinning}

Since we use results on the twinning property
for \fsts in this paper, we clarify the definition
of twinning property for \fsts. In the core of the paper,
it is said that restricting the horizontal twinning property
to \fsts correspond to the usual twinning property of \fsts.
By ``usual'' we mean the following definition, taken from~\cite{DBLP:journals/tcs/BealC02}.



\begin{definition}[Twinning property for \fsts of~\cite{DBLP:journals/tcs/BealC02}]\label{def:tp1}

Let $T = (Q, I, F, \delta)$ be a reduced \fst. $T$ satisfies the twinning property if
for all $q_0,q'_0\in I$, for all $q,q'\in Q$,  for all words $u_1,v_1,w_1,u_2,v_2,w_2\in\Sigma^*$, if:
\[
q_0\ \xrightarrow{u_1/v_1}\ q\ \xrightarrow{u_2/v_2}\ q\qquad
q'_0\ \xrightarrow{u_1/w_1}\ q'\ \xrightarrow{u_2/w_2}\ q'
\]
Then either $v_2=w_2=\epsilon$, or the following holds:

$(i)$ $|v_2| = |w_2|$

$(ii)$ $v_1{(v_2)}^\omega = w_1{(w_2)}^\omega$
\end{definition}

Our twinning property for \fsts is obtained by restricting
the horizontal twinning property of \vpts to \fsts. By restricting
we mean the following:


\begin{definition}[Twinning property for \fsts of this paper]\label{def:tp2}
Let $T = (Q, I, F, \delta)$ be a reduced \fst. $T$ satisfies the twinning property if
for all $q_0,q'_0\in I$, for all $q,q'\in Q$,  for all words $u_1,v_1,w_1,u_2,v_2,w_2\in\Sigma^*$, if:
\[
q_0\ \xrightarrow{u_1/v_1}\ q\ \xrightarrow{u_2/v_2}\ q\qquad
q'_0\ \xrightarrow{u_1/w_1}\ q'\ \xrightarrow{u_2/w_2}\ q'
\]

Then $\Delta(v_1,w_1) = \Delta(v_1v_2,w_1w_2)$.
\end{definition}

The two definitions are equivalent, as shown by the next lemma:

\begin{lemma}
  Definitions~\ref{def:tp1} and~\ref{def:tp2} are equivalent.
\end{lemma}

\begin{proof}
  First suppose that Definition~\ref{def:tp1} holds. If $v_2=w_2=\epsilon$,
  then clearly $\Delta(v_1,w_1) = \Delta(v_1v_2,w_1w_2)$. Otherwise
  $|v_2| = |w_2|$ and $v_1{(v_2)}^\omega = w_1{(w_2)}^\omega$. Then
  necessarily $v_1\preceq w_1$ (i.e. $v_1$ is a prefix of $w_1$)
  or $w_1\preceq v_1$. Wlog suppose that
  $v_1\preceq w_1$, i.e. $w_1 = v_1w'_1$ for some $w'_1$.
  Therefore $\Delta(v_1,w_1) = (\epsilon, w'_1)$, and
  $\Delta(v_1v_2,w_1w_2) = \Delta(v_2,w'_1w_2)$.


  We now prove that $\Delta(v_2,w'_1w_2) = (\epsilon, w'_1)$.
  Since $v_1{(v_2)}^\omega = w_1{(w_2)}^\omega$, we have
  ${(v_2)}^\omega = w'_1{(w_2)}^\omega$. Therefore $v_2w'_1{(w_2)}^\omega =
  v_2^\omega = w'_1{(w_2)}^\omega$. Since $|v_2| = |w_2|$, we get
  $v_2w'_1 = w'_1w_2$, from which we have $\Delta(v_2,w'_1w_2) =
  \Delta(v_2,v_2w'_1) = (\epsilon, w'_1)$.



  Conversely, suppose that Definition~\ref{def:tp2} holds and
  $v_2w_2\neq\epsilon$. Since
  $\Delta(v_1,w_1) = \Delta(v_1v_2,w_1w_2)$, we have either
  $v_1\preceq w_1$ or $w_1\preceq v_1$. Wlog suppose that $v_1\preceq
  w_1$, i.e. $w_1 = v_1w'_1$ for some $w'_1$. Therefore we have:
  \[
  \Delta(v_1,w_1) = (\epsilon,w'_1) = \Delta(v_1v_2,w_1w_2) = \Delta(v_2,w'_1w_2)
  \]
  Consequently, $v_2\preceq w'_1w_2$, and in particular, $w'_1w_2 =
  v_2w'_1$, which gives us the following series of equalities:
  \[
  w_1{(w_2)}^\omega = v_1w'_1{(w_2)}^\omega = v_1v_2w'_1{(w_2)}^\omega =
  v_1{(v_2)}^2w'_1{(w_2)}^\omega = \cdots = v_1{(v_2)}^\omega\qquad
  \]
\end{proof}


\subsection{HTP is decidable}\label{sec:htpdecidable}


\begin{lemma}\label{lem:not-htp}
Let $T$ be an \fvpt, $T$ does not satisfy the HTP if and only if
there exist $q_0,q'_0\in I$, $q,q'\in Q$, $\sigma, \sigma'\in\Gamma^*$
and $u_1,v_1,w_1,u_2,v_2,w_2\in\Sigma^*$, with either $v_2\neq \epsilon$ or $w_2\neq \epsilon$ and:
\[
(q_0,\bot) \ \xrightarrow{u_1/v_1}\ (q,\sigma)\ \xrightarrow{u_2/v_2}\ (q,\sigma)\qquad
(q'_0,\bot) \ \xrightarrow{u_1/w_1}\ (q',\sigma')\ \xrightarrow{u_2/w_2}\ (q',\sigma')
\]
and either $(i)$ $|v_2|\neq|w_2|$ or  $(ii)$ $|v_2|= |w_2|$, $|v_1|\leq |w_1|$ and  $v_1v_2\not\preceq w_1w_2$.
\end{lemma}
\begin{proof}
Let suppose that there exist $q_0,q'_0\in I$, $q,q'\in Q$, $\sigma, \sigma'\in\Gamma^*$
and $u_1,v_1,w_1,u_2,v_2,w_2\in\Sigma^*$, with either $v_2\neq \epsilon$ or $w_2\neq \epsilon$ and:
\[
(q_0,\bot) \ \xrightarrow{u_1/v_1}\ (q,\sigma)\ \xrightarrow{u_2/v_2}\ (q,\sigma)\qquad
(q'_0,\bot) \ \xrightarrow{u_1/w_1}\ (q',\sigma')\ \xrightarrow{u_2/w_2}\ (q',\sigma')
\]

And let show that if $(i)$ or $(ii)$ hold so does  $\del(v_1,w_1)\neq \del(v_1v_2,w_1w_2)$.

First suppose that $(i)$ holds.
Let $x=v_1\wedge w_1$ and $z=v_1v_2\wedge w_1w_2$, clearly there exists $y\in\Sigma^*$
 such that $z=xy$. By definition, we have $\del(v_1,w_1)=(x^{-1}v_1,x^{-1}w_1)$ and
 $\del(v_1v_2,w_1w_2)=({(xy)}^{-1}v_1v_2,{(xy)}^{-1}w_1w_2)$. Therefore if~$(i)$ holds then either
 $|x^{-1}v_1|\neq |{(xy)}^{-1}v_1v_2|$ or $|x^{-1}w_1|\neq |{(xy)}^{-1}w_1w_2|$.
 Indeed, suppose the first inequality does not hold,
 we have $|x^{-1}v_1|= |v_1|-|x| = |{(xy)}^{-1}v_1v_2| = |v_1|+|v_2|-|x|-|y|$,
 that is $0=|y|-|v_2|$. Therefore one can check that the second inequality must hold.
 We have shown that $(i)$ implies $\del(v_1,w_1)\neq \del(v_1v_2,w_1w_2)$.

Now, suppose $(ii)$ holds and let us show that we also have $\del(v_1,w_1)\neq \del(v_1v_2,w_1w_2)$.
We have $(ii)$ $|v_2|= |w_2|$, $|v_1|\leq |w_1|$ and $v_1v_2\not \preceq w_1w_2$.
Note that for any $u,v, x, y\in\Sigma^*$ with $\del(u,v)=(x,y)$ we have $u\not\preceq v$ if and only if
$x\neq \epsilon$ and $y\neq \epsilon$.
Therefore, if we pose $(y_1,y_2)=\del(v_1v_2,w_1w_2)$, we have,
by hypothesis, $v_1v_2\not \preceq w_1w_2$ and so $y_1\neq \epsilon$ and $y_2\neq \epsilon$.
Let pose $(x_1,x_2)=\del(v_1,w_1)$, if $(x_1,x_2)=(y_1,y_2)$ then $x_1\neq \epsilon$ and $x_2\neq \epsilon$,
that is $v_1\not\preceq w_1$, but then $\del(v_1v_2,w_1w_2)=\del(v_1,w_1)\cdot (v_2,w_2)$
which cannot be equal to $\del(v_1,w_1)$ (because, by hypothesis, one of $v_2$ and $w_2$ is not the empty word).

Now let suppose the HTP does not hold and let show that $(i)$ or $(ii)$ is satisfied for some words (as above).
So there exist $q_0,q'_0\in I$, $q,q'\in Q$, $\sigma, \sigma'\in\Gamma^*$
and $u_1,v_1,w_1,u_2,v_2,w_2\in\Sigma^*$ with:
\[
(q_0,\bot) \ \xrightarrow{u_1/v_1}\ (q,\sigma)\ \xrightarrow{u_2/v_2}\ (q,\sigma)\qquad
(q'_0,\bot) \ \xrightarrow{u_1/w_1}\ (q',\sigma')\ \xrightarrow{u_2/w_2}\ (q',\sigma')
\]
  such that $\del(v_1,w_1)\neq \del(v_1v_2,w_1w_2)$.
  Moreover, let us suppose, by contradiction, that for all $k\in\mathbb{N}$, if we replace $u_2$ by ${u_2}^k$
  (and thus $v_2$ and $w_2$ are replaced by ${v_2}^k$ and ${w_2}^k$ respectively),
   we get a system such that neither $(i)$ nor $(ii)$ do hold, that is
   for all $k\in\mathbb{N}$ we have
   $|{v_2}^k|= |{w_2}^k|$, $|v_1|\leq |w_1|$ and  $v_1{v_2}^k\preceq w_1{w_2}^k$.
   We now prove that this implies  $\del(v_1,w_1)= \del(v_1v_2,w_1w_2)$, which is a contradiction with the hypothesis.
    On the one hand, if for all $k$ we have $v_1{v_2}^k\preceq w_1{w_2}^k$ then we have $w_1 = v_1 {v_2}^a v'_2$ for some $a\in\mathbb N$ and some
   $v'_2\preceq v_2$. So, $\del(v_1,w_1)=\del(v_1,v_1 {v_2}^a v'_2)=(\epsilon, {v_2}^{a} v'_2)$.
   On the other hand,
    $v_1{v_2}^k\preceq w_1{w_2}^k$  and $|v_2|=|w_2|$ implies that we have $w_1w_2 = v_1 {v_2}^{a+1} v'_2$.
   So we have $\del(v_1v_2,w_1w_2)=\del(v_1v_2, v_1 {v_2}^{a+1} v'_2)=(\epsilon, {v_2}^{a} v'_2)$.
   Therefore $\del(v_1,w_1)= \del(v_1v_2,w_1w_2)$.
   This concludes the proof.
\end{proof}

\subsection{Proof of Theorem~\ref{thm:bm}}

Let $T$ be an \fvpt. We show that $\inter{T}$ is HBM iff $T$ satisfies
the HTP\@.


If $\inter{T}$ is HBM, then the HTP holds for $T$ by Lemma~\ref{lem:aa} (proved in this section). Conversely, if $T$ satisfies
the HTP, % and $T$ is reduced (which we assume in this paper),
then we apply Lemma~\ref{lm:HTP-delay} (proved this section) which
bounds the maximal difference between outputs of $T$, and then
Proposition~\ref{prop:complexity-eval} gives the complexity of the
evaluation algorithm.

\iffalse%
\fbox{PA\@: reprendre cette partie (reduced\ldots)}

If $T$ is not reduced, we cannot apply Lemma~\ref{lm:HTP-delay}
directly but we first have to reduce $T$ into $T_r$ while preserving the
satisfiability of the HTP\@. Let $q_1,\dots,q_n$ be the state
of $T$ and $F$ be the set of accepting states of $T$. It is well-known
that we can construct deterministic finite-state automata $A_{q_1},\dots, A_{q_n}$ over
the stack alphabet $\Gamma$ such that for all $q\in Q$, a stack
content $\sigma\in\Gamma^*$ is accepted by $A_q$ iff the configuration
$(q,\sigma)$ is co-accessible~\cite{springerlink:10.1007/3-540-13345-3_17}.
The reduction step is then easy. It suffices to enrich the state space
of $T$ with co-accessibility
information. In particular, if $Q_q$ is the set of states of $A_q$ for
all $q\in Q$, then the set of states of $T_r$ is $Q\times
Q_{q_1}\times \cdots \times Q_{q_n}$. The stack alphabet is also of the form
$\Gamma\times Q_{q_1}\times\cdots\times Q_{q_n}$. We give only an
informal explanation of this construction. When a run has reached the
configuration $((q,p_1,\dots,p_n), \sigma)$, it means that $T$ has
reached the configuration $(q,\sigma)$ and for all $i$, the automaton
$A_{q_i}$ is in state $q_i$ after reading $\sigma$, with the following
invariant (which ensures that $T_r$ is reduced): let $j$ be such that
$q = q_j$, then $p_j$ is an accepting state of $A_j = A_q$. On a call
symbol, a copy of the states of the automata $A_q$ before reading the
call symbol have to be stored on the stack so that when reading the
matching return, the states of the automata $A_q$ can be restored (and
again if $q_j$ is the state reached by $T_r$ after reading the return
symbol then we have to check whether $p_j$ is an accepting state).


The transducer $T$ can be obtained from $T_r$ by projecting on the
first component, and therefore it is clear that $T_r$ satisfies the
HTP whenever $T$ satisfies it.
\fi




\begin{lemma}\label{lem:aa}
  Let $T$ be an \fvpt. If $\inter{T}$ is HBM, then the HTP holds
  for $T$.
\end{lemma}

\begin{proof}
  By definition of HBM and BM, if $\inter{T}$ is HBM and there
  exists $K\in\Nat$ such that for all $u\in\dom(T)$, $h(u)\leq
  K$, then $\inter{T}$ is BM\@.


  Now suppose that the HTP does not hold for $T$. Therefore there are words
  $u_1,u_2,u_3,u'_3,v_1,v_2,v_3,w_1,w_2,w_3,w_3\in\Sigma^*$, stacks
  $\sigma,\sigma'$ and states $q,q'\in Q$, $q_0,q'_0\in I$ and
  $q_f,q'_f\in F$ such that:
  \[
  \left\{\begin{array}{llllllll}
  (q_0,\bot) & \xrightarrow{u_1/v_1} & (q,\sigma) &  \xrightarrow{u_2/v_2} &
  (q,\sigma) & \xrightarrow{u_3/v_3} & (q_f,\bot)\\

  (q'_0,\bot) & \xrightarrow{u_1/w_1} & (q',\sigma') &  \xrightarrow{u_2/w_2} &
  (q',\sigma') & \xrightarrow{u'_3/w_3} & (q'_f,\bot)\\
  \end{array}\right.
  \]
  and $\del(v_1,w_1) \neq \del(v_1v_2,w_1w_2)$. Let $K =
  \text{max}(h(u_1u_2u_3),h(u'_1u'_2u'_3))$. By definition of
  $\fst(T,K)$ (states are configurations of $T$) and of the twinning
  property for \fsts, the twinning property for \fsts does not hold for $\fst(T,K)$. Therefore
  $\fst(T,K)$ is not sequentializable~\cite{DBLP:journals/tcs/Choffrut77}
  and by Proposition~\ref{prop:bmfst}
  $\inter{\fst(T,K)}$ is not BM\@. Therefore $\inter{T}$
  is not HBM, otherwise $\inter{T}$ could be evaluated in space
  complexity $f(h(u))$ on any input word $u$, for some function
  $f$. That corresponds to bounded memory if we fix the height of the
  words to $K$ at most.
\end{proof}

For the converse, we can apply the evaluation algorithm of Section~\ref{sec:algo}, whose complexity depends on the maximal delay between
all the candidate outputs of the input word. We first prove that this
maximal delay is exponentially bounded by the
height of the word.

\iffalse%
\ms{PA match notations with those of the algorithm} Given a word $u$
prefix of a word in the domain of $T$, we define the maximal possible
output after reading $u$ as $Pref^T(u)=\bigwedge\{v \mid \exists
(i,\bot)\xrightarrow{u|v}(q,\sigma) \text{ co-reachable in }T\}$.
Then, the evaluation algorithm stores, after reading u, the set
$Reach(u)=\{(q,\sigma,w)\mid \exists
(i,\bot)\xrightarrow{u|v}(q,\sigma) \text{ co-reachable in }T \text{
  s.t. } v=Pref^T(u).w\}$.
\fi

\begin{lemma}\label{lm:HTP-delay}
  Let $T$ be an  \fvpt. If the HTP holds for $T$, then for all
  $s\in\Sigma^*$ we have $\maxoutdiffT(s) \leq {(|Q|\cdot|\Gamma|^{h(s)})}^2 M$, where
  $M=\max \{|t| \hmid (q,a,t,\gamma,q')\in\delta\}$.
%  prefix of a word in $Dom(T)$, and any tuple $(q,\sigma,w)\in
%  Reach(u)$, we have $|w| \leq (|Q|\cdot|\Gamma|^{h(u)})^2 M$, where $M$
%  denotes the maximal length of output words in $T$.
\end{lemma}

\begin{proof}
  Let $s\in\Sigma^*$. We consider two cases. We first assume that
  $s\in \dom(T)$. Let $u\in \Sigma^*$ be a prefix of $s$, we will
  prove that $\maxoutdiff(u) \leq {(|Q|\cdot|\Gamma|^{h(u)})}^2 M$.  Note
  that there exist $N = |Q|\cdot|\Gamma|^{h(u)}$ configurations reachable
  by words of height less than $h(u)$.  The proof is similar to that
  of~\cite{DBLP:journals/tcs/BealC02} for FST\@. It proceeds by
  induction on the length of $u$. If $|u|\leq N^2$, then the result is
  trivial. Otherwise, assume that $|u|>N^2$ and let $(q,\sigma,w),
  (q',\sigma',w')\in Q\times \Gamma^*\times \Sigma^*$ such that
  there exist runs
%  By definition of
%  $Reach(u)$, there exist another\msmanu{this element can be the same
%    as $(q,\sigma,w)$, for instance if $|Reach(u)|=1$, in which case
%    $w=\epsilon$. Maybe say just say ``there exists
%    $(q',\sigma',w')$}element $(q',\sigma',w')\in Reach(u)$ such that
%  $w\wedge w'=\varepsilon$.  There exist two runs associated with
%  these tuples:
  $\rho: (i,\bot)\xrightarrow{u|v}(q,\sigma)$ and $\rho':
  (i',\bot)\xrightarrow{u|v'}(q',\sigma')$, with $i,i'\in I$, $v = \lcpin u
  T\cdot w$, $v' = \lcpin u T\cdot w'$, and such that $\maxoutdiff(u) = |w|$. As
  $|u|>N^2$, we can decompose these two runs as follows:
  \[
  \left\{\begin{array}{llllllllll} \rho: (i,\bot) &
      \xrightarrow{u_1/v_1} & (q_1,\sigma_1) & \xrightarrow{u_2/v_2} &
      (q_1,\sigma_1) & \xrightarrow{u_3/v_3} & (q,\sigma) \\

  \rho': (i',\bot) & \xrightarrow{u_1/v'_1} & (q'_1,\sigma'_1) &  \xrightarrow{u_2/v'_2} &
  (q_1',\sigma_1') & \xrightarrow{u_3/v_3'} & (q',\sigma') \\
\end{array}\right.
\quad
\]
In addition, we have $u=u_1u_2u_3$, $u_2\neq\varepsilon$,
$v=\lcpin u T\cdot w = v_1v_2v_3$, and $v'=\lcpin u T\cdot w' = v_1'v_2'v_3'$.
Indeed, by the choice of $N$, there must exist a pair of
configurations that occurs twice. By the HTP property, we obtain
$\del(v_1v_2,v_1'v_2')=\del(v_1,v_1')$. By Lemma~\ref{lem:assocdelay} (see
Appendix~\ref{app:tp-relation}), this entails the equality
$\del(v_1v_2v_3,v_1'v_2'v'_3)
=\del(\del(v_1v_2,v_1'v_2')\cdot (v_3,v_3'))
=\del(\del(v_1,v_1')\cdot (v_3,v_3'))
=\del(v_1v_3,v_1'v'_3)$.  Thus, we obtain
$\del(w,w')=\del(v,v')=\del(v_1v_2v_3,v_1'v_2'v_3')=\del(v_1v_3,v_1'v_3')$. As
$v_1v_3$ and $v'_1v'_3$ are possible output words for the input word
$u_1u_3$, whose length is strictly smaller than $|u|$, we obtain $|w|
\leq \maxoutdiff(u_1u_3)$ and the result holds by induction.



We now consider the second case: $s\not\in\dom(T)$. Let $s'$ be the
longest prefix of $s$ such that there exists $s''$ such that
$s's''\in\dom(T)$. Since $T$ is reduced (w.l.o.g., as explained in
preliminaries), $s'$ correspond to the longest prefix of $s$ on which
there exist a run of $T$. Therefore we have $\maxoutdiffT(s) \leq
\maxoutdiffT(s')$ and we can apply the proof of the first case (as
$s'$ is a prefix of a word that belongs to $\dom(T)$) and we get
$\maxoutdiffT(s')\leq {(|Q|\cdot|\Gamma|^{h(s')})}^2 M$. Moreover,
$h(s')\leq h(s)$, therefore $\maxoutdiffT(s) \leq \maxoutdiffT(s')
\leq {(|Q|\cdot|\Gamma|^{h(s)})}^2 M$ and we are done.
\end{proof}


\section{Quadratic Height Bounded Memory Evaluation}%
\label{apx:TP}

\subsection{Decidability of the matched twinning property}%
\label{sec:apx-twinning}

\begin{proof}[Lemma~\ref{thm:decidability}]
  Let $T$ be a \fvpt. We construct in polynomial time a pushdown
  automaton with $s$ counters~\footnote{The number $s$ does not depend
    on the transducer $T$.} (one reversal) that accepts any word
  $u=u_1u_2u_3u_4$ that satisfies the premise of the \MTP but such that
  $\del(v_1v_3,w_1w_3) \neq \del(v_1v_2v_3v_4,w_1w_2w_3w_4)$ (i.e., the
  \MTP is not verified).  Therefore the \MTP holds if and only if no word
  is accepted by the automaton.  This can be checked in \conptime~\cite{vpts10}.


  The automaton simulates any two runs, and guesses the decomposition
  $u_1u_2u_3u_4$ (it checks that the decomposition is correct by
  verifying that each run is in the same state after reading $u_1$ and
  $u_2$, and in the same state after reading $u_3$ and $u_4$). With
  two counters it can check that $|v_2v_4|=|w_2w_4|$, if it is not the
  case then it accepts $u$ (indeed the \MTP is therefore not verified).
  The automaton checks that $\del(v_1v_3,w_1w_3) \neq
  \del(v_1v_2v_3v_4,w_1w_2w_3w_4)$ with the hypothesis (checked in
  parallel) that $|v_2v_4|=|w_2w_4|$. Let $A,B,C,D$ be four words with
  $A=a_1\dots a_l, B=b_1\dots b_m, C=c_1\dots c_n, D=d_1\dots d_p$,
  $l\geq m$. We show in Lemma~\ref{lm:delaymismatch} below, that
%two pairs of words (e.g. $A,B$ and
%  $C,D$ with $A=a_1\dots a_l, B=b_1\dots b_m, C=c_1\dots c_n,
%  D=d_1\dots d_p$, $l\geq m$) have different delays, that is
  $\del(A,B)\neq \del(C,D)$ holds if, and only if, at least one out of four
  simple conditions is true.  For example, the first condition states
  that there exists $k$ such that $a_{l-k} \neq b_{l-k}$ and either
  $(i)$ $k\geq |C|$, or $(ii)$ $c_{n-k}= d_{n-k}$.  The automaton
  guesses which condition holds and verifies it with the help of
  counters.

  We detail how to check the first condition, the others can be
  checked with the same technique.  The automaton guesses the value
  $k$ and with two counters verifies that $a_{l-k} \neq b_{l-k}$ as
  follows.  First it initializes both counters to $l-k$ (e.g., with an
  epsilon loop that increments both counters).  Then it counts the
  letters of both words $A$ and $B$ up to $l-k$ and
  records $a_{l-k}$
%(the $l-k$-th letter of $v_1v_3$)
  and $b_{l-k}$ and verifies that they are not equal.  Finally it must
  verify that either $(i)$ or $(ii)$ is satisfied.  The verification
  of $(i)$ is easy.
% But $(i)$ cannot
%  hold as $A=v_1v_3$ and $C= v_1v_2v_3v_4$ and $k \leq|A|$.
  To verify $(ii)$, i.e. $c_{n-k}= d_{n-k}$, it uses two additional
  counters and proceeds similarly as for checking $a_{l-k} \neq
  b_{l-k}$, but checks equality instead of inequality.
\end{proof}








\begin{lemma}\label{lm:delaymismatch}
  Let $A,B,C,D\in\Sigma^*$, such that $A=a_1\dots a_l, B=b_1\dots b_m,
  C=c_1\dots c_n, D=d_1\dots d_p$, and $l-m=n-p\ge 0$.
  %
  We have that $\del(A,B)\neq \del(C,D)$ if and only if one of the
  following conditions is satisfied:

\begin{enumerate}
%1
\item there exists $k$ such that $a_{l-k} \neq b_{l-k}$ and either $(i)$ $k\geq |C|$, or $(ii)$ $c_{n-k}= d_{n-k}$;
%2
\item there exists $k$ such that $c_{n-k}\neq d_{n-k}$ and either $(i)$ $k\geq |A|$, or $(ii)$ $a_{l-k} = b_{l-k}$;
%3
\item there exists $k$ such that $a_{l-k} \neq c_{n-k}$ and either
$(i)$ $k<l-m$, or
$(ii)$ there exists $k'$ with $a_{k'}\neq b_{k'}$ and $k+k'\leq l$;
%4
\item there exist $k,k'$ such that $b_{m-k} \neq d_{p-k}$ and $a_{k'}\neq b_{k'}$ and $k+k'\leq m$.
\end{enumerate}
\end{lemma}

\begin{proof}

  Let us define $E=A\wedge B$ and $F=C\wedge D$, and also
  $A',B',C',D'\in\Sigma^*$ such that $A=EA', B=EB', C=FC'$ and
  $D=FD'$, i.e. $(A',B')= \del(A,B)$ and $(C',D')= \del(C,D)$.


We first prove that each condition implies $\del(A,B)\neq \del(C,D)$,
i.e., that $(A',B')\neq(C',D')$.
If $|A'|\not=|C'|$ or $|B'|\not=|D'|$ then the result is immediate.
Now, assume that $|A'|=|C'|$ and $|B'|= |D'|$.
\begin{enumerate}
%1
\item By hypothesis we have
  $a_{l-k}\neq b_{l-k}$ therefore $|A'|\geq k+1$ (as $a_{l-k}\in A'$)
  and $|B'|\geq k+1-(l-m)$ (as $b_{l-k}\in B'$). Thus $|C'|\geq k+1$
  and $|D'|\geq k+m-l+1$. In particular, this implies that we are in
  case $(ii)$ as $|C|\geq |C'|\geq k+1$. We consider two cases: $(a)$
  if $a_{l-k} \neq c_{n-k}$ we have $A'\neq C'$ (because $a_{l-k}\in
  A'$ and $c_{n-k}\in C'$ and are at the same position in $A'$ and
  $C'$ as $|A'|=|C'|$), or $(b)$ if $a_{l-k} = c_{n-k}$ this means
  that $b_{l-k} \neq d_{n-k}$ (because $a_{l-k} \neq b_{l-k}$ and
  $c_{n-k}= d_{n-k}$), and so $B'\neq D'$ (because $b_{l-k} \in B'$
  and $d_{n-k}\in D'$ because $|B'|=|D'|$).
%2
\item Similar to proof of 1.
%3
\item We prove that condition $(i)$ implies $\del(A,B)\neq \del(C,D)$.
  Condition $(ii)$ is proved similarly.
% \ms{Olivier: should be written}.
  We know that $|A'|\geq |A|-|B|=l-m>k$ therefore $a_{l-k}\in A'$.
  Similarly, $|C'|=|A'|>k$, so $c_{n-k}\in C'$.
  By hypothesis $a_{l-k} \neq c_{n-k}$, therefore, as $|A'|=|C'|$,
  $A'$ and $C'$ differ on their $k$th letter from the right.
%4
\item Similar to proof of 3.
\end{enumerate}

Now suppose that $\del(A,B)\neq \del(C,D)$ and let us show that one of
the conditions is satisfied. First note that if $B'=\varepsilon$, then
$B$ is a prefix of $A$, and thus $|A'|=l-m$. In particular, we obtain
$|A'| \leq |C'| \leq |C|$. We call this property
$(\dagger_B)$. Similarly, $D'=\varepsilon$ entails $|C'| \leq |A'|
\leq |A|$, what we denote by $(\dagger_D)$.

We prove the property by considering several cases:
\begin{itemize}
\item $|A'|>|C|$: take $k=|A'|-1$, we have $a_{l-k} \neq
  b_{l-k}$. Note that $b_{l-k}$ does not exist iff $l-k>m$,
  \emph{i.e.} $B'=\varepsilon$. By property $(\dagger_B)$, this can
  not occur.  In addition, by definition of $k$, we have $k\geq |C|$
  and thus condition $1.(i)$ is satisfied.
%  \ms{Olivier: what happens if
%    $B'=\emptyword$? $b_{l-k}$ is undefined. This situation is not
%    clear, even in the lemma statement.} and $k\geq |C|$ (condition
%  $1.(i)$ is satisfied).
\item $|C'|>|A|$: take $k=|C'|-1$, we have $c_{n-k}\neq d_{n-k}$ (as
  above, $(\dagger_D)$ ensures that $d_{l-k}$ is well defined) and
  $k\geq |A|$: condition $2.(i)$ is satisfied.
\item
  $|A'|\leq|C|$ and $|C'|\leq|A|$:
  \begin{itemize}
  \item $|A'| > |C'|$ (this implies $|B'| > |D'|$): take $k=|A'|-1$,
    we have $a_{l-k} \neq b_{l-k}$ and $c_{n-k}= d_{n-k}$ (existence
    of $b_{l-k}$ and $d_{n-k}$ is ensured by $(\dagger_B)$ and
    $(\dagger_D)$): condition $1.(ii)$ is satisfied.
  \item $|C'| > |A'|$ (this implies $|D'| > |B'|$): take $k=|C'|-1$,
    then condition $2.(ii)$ is satisfied.
  \item $|A'|=|C'|$ (this implies $|B'|=|D'|$), we suppose $A'\neq C'$
    and prove that condition $3$ holds (the case $B'\neq D'$ is similar
    with condition $4$ holding).  Because $A'\neq C'$ and they have the
    same size, there must be a $k<|A'|$ with $a_{l-k} \neq c_{n-k}$, we
    consider two cases:
    \begin{itemize}
    \item $|A'|\leq|A|-|B|$, this implies that $k<|A|-|B|= l-m$
      therefore condition $3.(i)$ is satisfied.
    \item $|A'|> |A|-|B|$, take $k'=l-|A'|+1$ (the first position of
      $A'$ in $A$). Then we have $a_{k'}\neq b_{k'}$ and thus
      condition $3.(ii)$ is satisfied.
    \end{itemize}
  \end{itemize}
\end{itemize}
\end{proof}


\input{tp-relation}


\subsection{Proof of Theorem~\ref{thm:polyhbm}}


We can use the same proof as the proof of back direction of
Theorem~\ref{thm:bm}, the only difference is the lemma that bounds
the maximal difference between outputs of $T$.
%In the proof of Theorem
%\ref{thm:bm}, we also needed preservation of satisfiability of the HTP
%under reduction of the \vpt. This is also the case for the \MTP.

We prove the following lemma, which states that the \MTP implies
that in the evaluation algorithm,
the delays stored by the algorithm can be bounded linearly in the
height of the input word.


\begin{lemma}\label{lem:boundedvertical}
  Let $T$ be an \fvpt. If the \MTP holds for $T$, then for any
  word $s \in \Sigma^*$, we have
%  and any tuple
%  $(q,\sigma,w)\in Reach(u)$, we have $|w| \leq
  $\maxoutdiffT(s) \leq   (h(s)+1) \cdot  \left (
    {(|Q|\cdot |\Gamma|^{|Q|^4})}^2+1 \right ) \cdot  M$, where   $M=\max \{|t|
  \hmid (q,a,t,\gamma,q')\in\delta\}$.
\end{lemma}

% TEMP
\begin{proof}
  Let $s\in\Sigma^*$. We assume that $s\in\dom(T)$ (we can handle the
  case $s\not\in\dom(T)$ as in the proof of Lemma~\ref{lm:HTP-delay}
  for the HTP).
  %
  Consider a word $u$ prefix of $s$. There exists a
  unique decomposition of $u$ as follows:
  $
  u = u_0 c_1 u_1 c_2 \ldots u_{n-1} c_n u_n
  $,
  where $n=\hc(u)$ (the current height of $u$),
  and for any $i$, we have $c_i\in \Sigma_c$ and
  $u_i$ is well-nested.  Indeed, as $n=\hc(u)$, the word $u$ contains
  exactly $n$ pending calls, that correspond to $c_i$'s, and other
  parts of $u$ can be gathered into well-nested words.

  If each of the $u_i$'s is such that $|u_i| \leq
  {(|Q|\cdot |\Gamma|^{|Q|^4})}^2$, then the property holds as length of word
  $u$ can be bounded by $(\hc(u)+1) \cdot  \left (
    {(|Q|\cdot |\Gamma|^{|Q|^4})}^2+1 \right )$.

  Otherwise, we prove that there exists a strictly shorter input word
  that produces the same delays as $u$ when evaluating the
  transduction on it. Therefore, consider a word $w$ such that
  $(q_0,\bot)\xrightarrow{u/w}{(q,\sigma)}$ for some $q_0\in I$. Then
  there exist runs $\varrho$, $\varrho'$ in $T$ producing respectively
  as output words $v$ and $v'$, such that $v = (v\wedge v') \cdot  w$.
  Consider the smallest index $i$ such that $|u_i| >
  {(|Q|\cdot |\Gamma|^{|Q|^4})}^2$. We distinguish two cases:
  \begin{enumerate}
  \item if $h(u_i)\leq |Q|^4$, then we can reduce the length of $u_i$
    using the HTP by exhibiting two
    configurations occurring twice in runs $\varrho$ and
    $\varrho'$. This yields an input word $u'$, strictly shorter than
    $u$, that produces the same delays as $u$ (see the proof of
    Lemma~\ref{lm:HTP-delay}).
  \item if $h(u_i) > |Q|^4$, then we prove that we can ``pump
    vertically'' $u_i$, and then reduce its length too. Indeed, let
    $k$ be the first position in word $u_i$ at which height $h(u_i)$
    is obtained. As $u_i$ is well-nested, we can define for each
    $0\leq j < h(u_i)$ the unique position $\Left{j}$
    (resp. $\Right{j}$) as the largest index, less than $k$ (resp.\ the
    smallest index, larger than $k$), whose height is $j$ (see
    Figure~\ref{fig:vertical}). As $h(u_i) > |Q|^4$, there exist two
    heights $j$ and $j'$ such that configurations reached at positions
    $\Left{j}$, $\Left{j'}$, $\Right{j}$ and $\Right{j'}$ in runs
    $\varrho$ and $\varrho'$ satisfy the premises of the matched twinning
    property, considering the prefix $u_0 c_1 \ldots c_i u_i$ of
    $u$. Thus, one can replace in this prefix $u_i$ by a shorter word
    $u'_i$ and hence reduce its length, while preserving the delays
    reached after it. Let $u'$ be the word obtained from $u$ by
    substituting $u'_i$ to $u_i$, hence $|u'|<|u|$. By
    Lemma~\ref{lem:assocdelay}, this entails that the delays reached
    after $u$ and $u'$ are the same, proving the result.
  \end{enumerate}

\end{proof}

\input{figvertical}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> tp-relation.tex <==
\section{Combinatorial results}\label{app:tp-relation}
%\subsection{\MTP is preserved by equivalent transducers}


\ignore{

In this section we prove Theorem~\ref{thm:eqrelation}.
%
We extend the concatenation to pairs of words and denote it by
$\cdot$, i.e. $(u,v)\cdot (u',v') = (uu',vv')$.

\paragraph*{Proof of Theorem~\ref{thm:eqrelation}}

\begin{proof}
  We assume that $T_1$ is not twinned and show that $T_2$ is not
  twinned either. By definition of the \MTP there are two runs of the
  form
  \[
  \left\{\begin{array}{llllllllllllllllll}
  (i_1,\bot) & \xrightarrow{u_1|v_1} & (p_1,\sigma_1) &  \xrightarrow{u_2|v_2} &
  (p_1,\sigma_1\beta_1) &  \xrightarrow{u_3|v_3} & (q_1,\sigma_1\beta_1) &
  \xrightarrow{u_4|v_4} & (q_1,\sigma_1) \\

  (i_1',\bot) & \xrightarrow{u_1|v'_1} & (p_1',\sigma_1') &  \xrightarrow{u_2|v'_2} &
  (p_1',\sigma_1'\beta'_1) &  \xrightarrow{u_3|v'_3} & (q_1',\sigma_1'\beta'_1) &
  \xrightarrow{u_4|v'_4} & (q'_1,\sigma'_1) \\
  \end{array}\right.
  \]
  such that $(q,\sigma_1)$ and $(q',\sigma'_1)$ are co-accessible and
  $\del(v_1v_3,v'_1v'_3) \neq \del(v_1v_2v_3v_4,v'_1v'_2v'_3v'_4)$.
  We will prove that by pumping the loops on $u_2$ and $u_4$
  sufficiently many times we will get a similar situation in $T_2$,
  proving that $T_2$ is not twinned. It is easy to show that there
  exist $k_2> 0$,  $k_1,k_3\geq 0$,
  $w_i,w'_i\in\Sigma^*$, $i\in\{1,\dots,4\}$,
  some states $i_2,p_2,q_2,i'_2,p'_2,q'_2$ of $T_2$ and some
  stack contents $\sigma_2,\beta_2,\sigma'_2,\gamma'_2$  of $T_2$ such that we
  have the following runs in $T_2$:%
%%   $$
%%   \left\{\begin{array}{llllllllllllllllll}
%%   (i_2,\bot) & \xrightarrow{\begin{array}{ll}u_1(u_2)^{k_1}/\\w_1(w_2)^{k_1}\end{array}} & (p_2,\sigma_2) &  \xrightarrow{\begin{array}{l}(u_2)^{k_2}/\\(w_2)^{k_2}\end{array}} &
%%   (p_2,\sigma_2\beta_2) &  \xrightarrow{\begin{array}{l}(u_2)^{k_3}u_3 (u_4)^{k_3}/\\(w_2)^{k_3}w_3(w_4)^{k_3}\end{array}} & (q_2,\sigma_2\beta_2) &
%%   \xrightarrow{\begin{array}{l}(u_4)^{k_2}/\\(w_4)^{k_2}\end{array}} & (q_2,\sigma_2) \\

%%   (i_2',\bot) & \xrightarrow{\begin{array}{ll}u_1(u_2)^{k_1}/\\w'_1(w'_2)^{k_1}\end{array}} & (p_2',\sigma_2') & \xrightarrow{\begin{array}{l}(u_2)^{k_2}/\\(w'_2)^{k_2}\end{array}} &
%%   (p_2',\sigma_2'\beta'_2) &  \xrightarrow{\begin{array}{l}(u_2)^{k_3}u_3 (u_4)^{k_3}/\\(w'_2)^{k_3}w'_3(w'_4)^{k_3}\end{array}} & (q_2',\sigma_2'\beta'_2) &
%%   \xrightarrow{\begin{array}{l}(u_4)^{k_2}/\\(w'_4)^{k_2}\end{array}} & (q'_2,\sigma'_2) \\
%%   \end{array}\right.$$
%%   %
%%   such that $(q_1,\sigma_1)$ and $(q_2,\sigma_2)$
%%   (resp. $(q'_1,\sigma'_1)$ and $(q'_2,\sigma'_2)$) are co-accessible
%%   with the same input word $u_5$ (resp. $u'_5$).
  \[
  \!\!\!\left\{\begin{array}{llllllllllllllllllllllllllllll}
  \!\!\! (i_2,\bot) \! &
  \!\xrightarrow{u_1u_2^{k_1}|w_1} \! &
  \!(p_2,\sigma_2) \! & \!
  \xrightarrow{u_2^{k_2}| w_2} \! & \!
  (p_2,\sigma_2\beta_2) \! & \!
  \xrightarrow{u_2^{k_3}u_3u_4^{k_3}|w_3} \! & \!
  (q_2,\sigma_2\beta_2) \! & \!
  \xrightarrow{u_4^{k_2}|w_4}\!  & \!
  (q_2,\sigma_2) \\

  \!\!\! (i_2',\bot) \! & \!
  \xrightarrow{u_1u_2^{k_1}|w'_1} \! & \!
  (p_2',\sigma_2') \! & \! \xrightarrow{
      u_2^{k_2}| w'_2} \! & \!
  (p_2',\sigma_2'\beta'_2) \! & \! \xrightarrow{
      u_2^{k_3}u_3u_4^{k_3}|w'_3} \! & \!
  (q_2',\sigma_2'\beta'_2) \! & \!
  \xrightarrow{u_4^{k_2}|w'_4} \! & \! (q'_2,\sigma'_2) \\
  \end{array}\right.
  \]
  such that $(q_1,\sigma_1)$ and $(q_2,\sigma_2)$ are co-accessible
  with the same input word $u_5$, and $(q'_1,\sigma'_1)$ and
  $(q'_2,\sigma'_2)$ are co-accessible with the same input word
  $u'_5$. Now for all $i\geq 0$, we let
  \[
  \begin{array}{llllllllll}
  V^{(i)} = v_1{(v_2)}^{k_1+ik_2+k_3} v_3
  {(v_4)}^{k_1+ik_2+k_3} & W^{(i)} = w_1{(w_2)}^{i}w_3{(w_4)}^i \\
  V'^{(i)} = v'_1{(v'_2)}^{k_1+ik_2+k_3} v'_3
  {(v'_4)}^{k_1+ik_2+k_3} & W'^{(i)} = w'_1{(w'_2)}^{i}w'_3{(w'_4)}^i \\
  D_1(i)  = \Delta(V^{(i)}, V'^{(i)}) & D_2(i) = \Delta(W^{(i)}, W'^{(i)})
  \end{array}
  \]
  In other words, $D_1(i)$ (resp. $D_2(i)$) is the delay in $T_1$
  (resp. $T_2$) accumulated on the input word
  $u_1{(u_2)}^{k_1+ik_2+k_3}u_3{(u_4)}^{k_1+ik_2+k_3}$ by the two runs of
  $T_1$ (resp. $T_2$).


  There is a relation between the words $V^{(i)}$ and
  $W^{(i)}$. Indeed, since $T_1$ and $T_2$ are equivalent and
  $(q_1,\sigma_1)$ and $(q_2,\sigma_2)$ are both co-accessible by the
  same input word, for all $i\geq 1$, either $V^{(i)}$ is a prefix of
  $W^{(i)}$ or $W^{(i)}$ is a prefix of $V^{(i)}$, i.e., there exist $X\in\Sigma^*$ such that:
  for all $i\geq 1$, $V^{(i)} = W^{(i)}X$ or for all $i\geq 1$
  $V^{(i)}X = W^{(i)}$. Similarly, there exists $X'\in\Sigma^*$ such that
  for all $i\geq 1$, $V'^{(i)} =
  W'^{(i)}X'$ or for all $i\geq 1$, $V'^{(i)}X' = W'^{(i)}$.


  We now prove the following key result: for all $i,j\geq 1$,
  \[
  D_1(i)\neq D_1(j)\implies D_2(i)\neq D_2(j)
  \]
  We consider two cases (the other ones being symmetric):
  \begin{itemize}
    \item for all $\ell\geq 1$, $V^{(\ell)} = W^{(\ell)}X$ and $V'^{(\ell)} =
      W'^{(\ell)}X'$. Then we have:
      \[
      \begin{array}{lllll}
        & \del(V^{(i)},V'^{(i)}) & \neq &  \del(V^{(j)},V'^{(j)}) \\
        \text{$\Rightarrow$ }
        & \del(W^{(i)}X,W'^{(i)}X') & \neq &  \del(W^{(j)}X,W'^{(j)}X') \\
        \text{$\Rightarrow$ }
        & \del(\del(W^{(i)},W'^{(i)})\cdot (X,X')) & \neq &
        \del(\del(W^{(j)},W'^{(j)})\cdot (X,X')) & \text{(Lemma~\ref{lem:assocdelay})}\\
        \text{$\Rightarrow$ }
        & \del(W^{(i)},W'^{(i)}) & \neq &
        \del(W^{(j)},W'^{(j)})
      \end{array}
      \]

    \item for all $\ell\geq 1$, $V^{(\ell)} = W^{(\ell)}X$ and
      $V'^{(\ell)}X' = W'^{(\ell)}$. Then we have:
      \[
      \begin{array}{lllll}
        & \del(V^{(i)},V'^{(i)}) & \neq &  \del(V^{(j)},V'^{(j)}) \\
        \text{$\Rightarrow$ }
        & \del(W^{(i)}X,V'^{(i)}) & \neq &  \del(W^{(j)}X,V'^{(j)}) \\
        \text{$\Rightarrow$ }
        & \del(\del(W^{(i)},V'^{(i)})\cdot (X,\epsilon)) & \neq &
        \del(\del(W^{(j)},V'^{(j)})\cdot (X,\epsilon)) & \text{(Lemma~\ref{lem:assocdelay})}\\
        \text{$\Rightarrow$ }
        & \del(W^{(i)},V'^{(i)}) & \neq &
        \del(W^{(j)},V'^{(j)}) \\
        \text{$\Rightarrow$ }
        & \del(\del(W^{(i)},V'^{(i)})\cdot (\epsilon, X'))  & \neq &
        \del(\del(W^{(j)},V'^{(j)})\cdot (\epsilon,X')) & \text{(Lemma~\ref{lem:eqdelay})} \\
        \text{$\Rightarrow$ }
        & \del(W^{(i)},V'^{(i)}X')  & \neq &
        \del(W^{(j)},V'^{(j)}X') & \text{(Lemma~\ref{lem:assocdelay})} \\
        \text{$\Rightarrow$ }
        & \del(W^{(i)},W'^{(i)})  & \neq &
        \del(W^{(j)},W'^{(j)}) &  \\

      \end{array}
      \]

  \end{itemize}


  Now by Lemma~\ref{lem:diffcont}, since $\Delta(v_1v_3,v'_1v'_3)\neq
  \Delta(v_1v_2v_3v_4,v'_1v'_2v'_3v'_3)$,  there exists
  $i_0\geq 1$ such that for all $i,j\geq i_0$, if $i\neq j$ then
  $\del(v_1{(v_2)}^{i}v_3{(v_4)}^i,v'_1{(v'_2)}^{i}v'_3{(v'_4)}^i)\neq
  \del(v_1{(v_2)}^{j}v_3{(v_4)}^{j},v'_1{(v'_2)}^{j}v'_3{(v'_4)}^{j})$.
  In particular since $k_2\geq 1$, we have $D_1(i)\neq D_1(j)$ for all
  $i,j\geq i_0$ and $i\neq j$. By the last intermediate result, we get
  $D_2(i_0)\neq D_2(i_0+1)$. Therefore the \MTP does not hold for $T_2$.
\end{proof}


\begin{lem}\label{lem:assocdelay}
  For all $u,u',v,v'\in\Sigma^*$, $\del(uu',vv') = \del(\del(u,v)\cdot (u',v'))$.
\end{lem}

\begin{proof}
  Let $X = uu'\wedge vv'$ and $Y = u\wedge v$. There exists $A,B,C,D$
  such that $A\wedge B=\epsilon$, $C\wedge D = \epsilon$, and:
  \[
  \begin{array}{l@{\quad}l}
    uu' = XA & u = YC \\
    vv' = XB & v = YD \\
    \del(uu',vv') = (A,B) & \del(u,v) = (C,D) \\
  \end{array}
  \]
  We have necessarily $|X| \geq |Y|$ since $X$ is the longest common % chktex 1
  prefix of $uu'$ and $vv'$ and $Y$ is the longest common prefix of
  $u$ and $v$. Now we have $YCu'=XA$ and $YDv' = XB$, i.e.
  $Cu' = Y^{-1}XA$ and $Dv' = Y^{-1}XB$. Since $A\wedge B=\epsilon$,
  we have $\del(Cu',Dv') = (A,B)$, i.e. $\del(\del(u,v)\cdot (u',v')) = (A,B) =
  \del(uu',vv')$.
\end{proof}

\begin{lem}\label{lem:eqdelay}
  For all $u,u',v,v',w,w'\in\Sigma^*$, we have
  \[
  \del(\del(u,u')\cdot (w,w')) = \del(\del(v,v')\cdot (w,w'))\text{ iff } \del(u,u')=\del(v,v')
  \]
\end{lem}

\begin{proof}
  There exists $A,B,C,D$ and $X,Y$ such that:
  \[
  \del(u,u')=(A,B)\quad \del(v,v')=(C,D)\quad u=XA\quad u'=XB\quad v=YC\quad v'=YD
  \]
  Let also $E,F,G,H$ such that $\del(Aw,Bw') = (E,F)$ and $\del(Cw,Dw') =
  (G,H)$. Clearly, if $A=C$ and $B=D$, we have $E=G$ and $F=H$.

  Conversely, suppose that $A\neq C$ (the case $B\neq D$ is
  symmetric). We show that $E\neq G$ or $F\neq H$. By definition of the delay, we know that $A\wedge B = \epsilon$, and
  $C\wedge D = \epsilon$. Therefore we have the following cases, for
  some words $A',B',C',D'$ and letters $a,b,c,d$ such that $a\neq b$
  and $c\neq d$:
  \begin{enumerate}
    \item $A = aA'$ and $B=bB'$, $C=cC'$ and $D=dD'$ for some
      $A',B',C',D'$. Therefore $\del(Aw,Bw') = (Aw,Bw') = (E,F)$ and $\del(Cw,Dw') =
      (Cw,Dw') = (G,H)$. Since $A\neq C$, we get $E\neq G$;

    \item $A = aA'$ and $B=bB'$, and $D=\epsilon$. Therefore
      $\del(Aw,Bw')= (Aw,Bw') = (E,F)$ and $\del(Cw,Dw') = \del(Cw,w') =
      (G,H)$. We have necessarily $|H|\leq |w'|$. Since
      $B\neq\epsilon$, we have $|F| = |Bw'| > |w'| \geq
      |H|$. Therefore $F\neq H$;

    \item $A = aA'$ and $B = bB'$ and $C=\epsilon$. We can apply the
      same argument as case 2;

    \item $A = \epsilon$ and $C = cC'$ and $D=dD'$. This case is
      symmetric to case $2$;

    \item $B = \epsilon$ and $C=cC'$ and $D=dD'$. This case is
      symmetric to case $2$;

    \item $A = \epsilon$ and $C = \epsilon$. This case is not possible
      since we have assumed $A\neq C$;

    \item $A = \epsilon$ and $D = \epsilon$ ($C\neq\epsilon$). We have
      $\del(Aw,Bw') = \del(w,Bw')$ and $\del(Cw,Dw') = \del(Cw,w')$. Suppose that
      $E = G$ and $F = H$. Then there exists $Z,Z'$ such that $w =
      ZE$, $Bw' = ZF$, $Cw = Z'E$ and $w' = Z'F$. Therefore
      $Bw' = BZ'F = ZF$, and $BZ' = Z$, so that $w = BZ'E$ and $Cw =
      CBZ'E = Z'E$, i.e. $CB = \epsilon$, which contradicts $C\neq
      \epsilon$;

    \item $B = \epsilon$ and $C = \epsilon$. This case is symmetric to
      the previous case;

    \item $B = \epsilon$ and $D = \epsilon$. Then we have
      $\del(Aw,Bw') = \del(Aw,w')$ and $\del(Cw,Dw') = \del(Cw,w')$. Again suppose
      that $E = G$ and $F = H$, therefore there exists $Z,Z'$ such
      that
      $Aw = ZE$, $w' = ZF$, $Cw = Z'E$ and $w' = Z'F$. Therefore $Z =
      Z'$, which implies $Aw = Cw$. This contradicts $A\neq C$.
  \end{enumerate}
\end{proof}

} % ignore

\olivier{je n'ai pas relu}

We prove Lemma~\ref{lem:diffcont}, used in the proof of
Proposition~\ref{prop:OBM-implies-MTP}.
We will need the following lemma.

\begin{lem}\label{lem:eqpref}
  Let $v_1,v_2,v_3,v_4,w_1,w_2,w_3,w_4\in\Sigma^*$ and for all $i\geq
  0$, let
  \[
  V^{(i)}  =  v_1{(v_2)}^{i}v_3{(v_4)}^i \qquad\qquad W^{(i)}  =  w_1{(w_2)}^{i}w_3{(w_4)}^i.
  \]
  If there exist $K\geq 0$ and $X\in \Sigma^*$ such that for all
  $i\geq K$, $V^{(i)} = W^{(i)} X$, then for all $i\geq 0$, $V^{(i)} =
  W^{(i)} X$.
\end{lem}

\begin{proof}
First note that we have $|v_2v_4|=|w_2w_4|$, this is a straight consequence from the fact that  for all $i\geq K$, $V^{(i)} = W^{(i)} X$.
We consider two cases:
\begin{itemize}
\item $|v_2|\neq |v_4|$: in that case we can show that the primitive roots
of $v_2,v_4, w_2,w_4$ are conjugate
(see for example~\cite{DBLP:journals/corr/abs-1002-1443})
and therefore have the same length.
Therefore we can apply Theorem 1 of~\cite{DBLP:journals/tcs/HolubK07} which yields the result.
\item $|v_2|=|v_4|$: in that case we also have $|w_2|=|w_4|$,
and suppose $|v_1|\geq|w_1|$ (the case $|v_1|<|w_1|$ is similar).
There exists $Y\in\Sigma^*$, such that for any $i\geq K$ we have
$v_1{v_2}^i=w_1{w_2}^i Y$ and $Yv_3{v_4}^i=w_3{w_4}^i X$.
 Therefore we can apply Theorem 2 of~\cite{DBLP:journals/tcs/HolubK07}
which shows that these equalities hold for any $i$.
 For any $i$ we have $V^{(i)}=v_1{v_2}^{i}v_3{v_4}^{i}=w_1{w_2}^{i} Yv_3{v_4}^{i}=w_1{w_2}^{i}w_3{w_4}^{i} X= W^{(i)} X$.
\end{itemize}
\end{proof}

\begin{lem}\label{lem:diffcont}
  Let $v_1,v_2,v_3,v_4,w_1,w_2,w_3,w_4\in\Sigma^*$ and for all $i\geq
  0$, let
  \[
  V^{(i)}  =  v_1{(v_2)}^{i}v_3{(v_4)}^i \qquad\qquad W^{(i)}  =  w_1{(w_2)}^{i}w_3{(w_4)}^i.
  \]
  If $\del(V^{(0)},W^{(0)})\neq \del(V^{(1)},W^{(1)})$, then there exists
  $i_0\geq 1$ such that for all $i,j\geq i_0$, if $i\neq j$
  then $\del(V^{(i)},W^{(i)})\neq \del(V^{(j)},W^{(j)})$.
\end{lem}

\begin{proof}
  First note that since $\del(V^{(0)},W^{(0)})\neq
          \del(V^{(1)},W^{(1)})$, we clearly have $|v_2v_4|\neq \epsilon$
          or $|w_2w_4|\neq\epsilon$,
  We write $u\preceq v$ if $u$ is a prefix of $v$, and
  $u||v$ if $u$ and $v$ are incomparable, i.e. $u\wedge v = \emptyword$.
  We consider several cases:

  \begin{itemize}
    \item[1.] there is $K\geq 1$ such that for all $i\geq K$,
      $V^{(i)}\preceq W^{(i)}$ or $W^{(i)} \preceq V^{(i)}$.
      Consider the lengths of $V^{(i)}$ and $W^{(i)}$.
      When $K$ is large enough,
      one of $V^{(i)}$ and $W^{(i)}$ is always the prefix of the other,
      for $i\ge K$: $V^{(i)}\preceq W^{(i)}$ if $|v_2v_4|\le|w_2w_4|$,
      and $W^{(i)}\preceq V^{(i)}$ otherwise.
      Let us assume that $|v_2v_4|\le|w_2w_4|$, i.e.,
      for all $i\geq K$, there exists
      $X_i$ such that $W^{(i)} = V^{(i)}X_i$.  The other case is
      symmetric.
      We have
      $|W^{(i+1)}| - |W^{(i)}| = |w_2w_4| =
      |V^{(i+1)}| + |X_{i+1}| - |V^{(i)}| - |X_i|$, i.e.
      $|w_2w_4| = |V^{(i)}| + |v_2v_4| + |X_{i+1}| - |V^{(i)}| - |X_i|$, i.e.
      $|X_{i+1}| - |X_i| = |w_2w_4| - |v_2v_4|$.
      We again consider several cases:
      \begin{itemize}
      \item[1.1] $|w_2w_4| > |v_2v_4|$. We
        have $|X_K| < |X_{K+1}| < |X_{K+2}| \ldots$, and by definition
        of the delay, $\del(V^{(i)},W^{(i)}) = (\epsilon,
        X_i)$. Therefore the delay always increases in size as $i$
        icreases and we get the result;


      \item[1.2] $|w_2w_4| = |v_2v_4|$. We show that this case is not
        possible. Indeed, it implies that $|X_{K}|
        = |X_{K+1}| = |X_{K+2}| \dots$. Therefore by definition of
        $V^{(i)}$ and $W^{(i)}$, there exists $K'\geq
        K$ and $X\in\Sigma^*$ such that $X = X_{K'} = X_{K'+1} = X_{K'+2}\dots$. By Lemma~\ref{lem:eqpref}, we get $W^{(0)} = V^{(0)}X$ and $W^{(1)} =
        V^{(1)}X$, which contradicts $\del(W^{(0)},V^{(0)})\neq \del(W^{(1)},V^{(1)})$.

      \end{itemize}

    \item[2.] for all $K\geq 1$, there is $i\geq K$ such that
      $V^{(i)}||W^{(i)}$. We show in this case that one of the two
      components of the delay always increases in size when $i$
      increases. We consider several cases depending on where the
      first difference between $V^{(i)}$ and $W^{(i)}$ occurs. The
      cases we consider also depend on $K$. In particular, by taking a
      large $K$ it can reduce the number of cases we have to consider.
      For some $\alpha_1,\alpha_2,\alpha_3\in\Sigma^*$ and $a,b\in\Sigma$ such
      that $a\neq b$, and for a $K$ large enough, one of the
      following condition holds:

      \begin{itemize}
        \item[2.1] there is $i\geq K$ such that
          $v_1{(v_2)}^i = \alpha_1a\alpha_2$ and $w_1{(w_2)}^i =
          \alpha_1b\alpha_3$, as illustrated below.

          \input{figcase2-1}

          Then for all $j\geq i$:
          \[
          \del(V^{(j)},W^{(j)}) = (a\alpha_2{(v_2)}^{j-i}v_3{(v_4)}^j, b\alpha_3{(w_2)}^{j-i}w_3{(w_4)}^j)
          \]
          Since $|v_2v_4|\neq \epsilon$ or $|w_2w_4|\neq \epsilon$, some of the two components of the delays is always
          increasing in size as $j$ icreases, which proves the result;


        \item[2.2] $w_2 = \epsilon$ and $v_1 = \alpha_1a\alpha_2$ and
          there is $i\geq K$ such that
          $w_1w_3{(w_4)}^i = \alpha_1b\alpha_3$, as illustrated below.

          \input{figcase2-2}

          Then for all $j\geq i$:
          \[
          \del(V^{(j)},W^{(j)}) = (a\alpha_1v_2^{j}v_3{(v_4)}^{j},
          b\alpha_3{(w_4)}^{j-i})
          \]
          Since $v_2v_4\neq\epsilon$ or $w_4\neq \epsilon$, one of the
          two components of the delays is always increaing in size;


        \item[2.3] there is $i\geq K$ such that $v_1{(v_2)}^i =
          \alpha_1a\alpha_2$ and $w_1{(w_2)}^{i}w_3 =
          \alpha_1b\alpha_3$, with $|\alpha_1|\geq |v_1|$ and $|\alpha_1|\geq |w_1{(w_2)}^i|$
          (otherwise it is case 2.1). We also assume that $w_2\neq
          \epsilon$ (otherwise it can be proved similarly as case
          2.1). Therefore $v_2\neq\epsilon$. This case is illustrated
          below:

          \input{figcase2-3}


          We have taken $K$ large enough, so that $v_2^i$ and
          $w_2^i$ have a common factor of length at least
          $|v_2|+|w_2|$. The strong theorem of Fine and Wilf~\cite{Lothaire97} implies that
          the primitive roots of $v_2$ and $w_2$ are
          conjugate: there are $t_1,t_2\in\Sigma^*$ and
          $n,p \geq 1$ such that $v_2 = {(t_1t_2)}^n$ and $w_2 =
          {(t_2t_1)}^p$. It can be shown (see for instance~\cite{DBLP:journals/corr/abs-1002-1443}) that we can choose
          $t_1$ and $t_2$ such that there exist $k_1,k_2\geq 0$ verifying:
          \[
          v_1 = (v_1\wedge w_1){(t_2t_1)}^{k_1}t_2\qquad w_1=(v_1\wedge w_1){(t_2t_1)}^{k_2}
          \]
          Let $\alpha'_1$ be such that $\alpha_1 =
          w_1{(w_2)}^i\alpha'_1$. There exist $k_3$, $X$ and
          $Y$ such that $\alpha'_1 = {(t_2t_1)}^{k_3}X$ with $t_2t_1 =
          XaY$, and $w_3 = \alpha_1'b\alpha_3$, as illustrated below
          (we assume that $|w_1| < |v_1|$ on the picture).


          \input{figcase2-3bis}

            We have for all $j\geq i$:
            \[
            \begin{array}{lllll}
              & & \del(V^{(j)},W^{(j)}) \\
              & = & \del(v_1{(v_2)}^{j}v_3{(v_4)}^j,w_1{(w_2)}^{j}w_3{(w_4)}^j)
              \\
              & = & \del((v_1\wedge w_1){(t_2t_1)}^{k_1}t_2{(t_1t_2)}^{jn}v_3{(v_4)}^j,w_1{(w_2)}^{j}w_3{(w_4)}^j) \\
              & = & \del((v_1\wedge w_1)t_2{(t_1t_2)}^{k_1+jn}v_3{(v_4)}^j,w_1{(w_2)}^{j}w_3{(w_4)}^j) \\
              & = & \del((v_1\wedge w_1)t_2{(t_1t_2)}^{k_1+jn}v_3{(v_4)}^j,(v_1\wedge w_1){(t_2t_1)}^{k_2}{(w_2)}^{j}w_3{(w_4)}^j) \\
              & = & \del(t_2{(t_1t_2)}^{k_1+jn}v_3{(v_4)}^j,{(t_2t_1)}^{k_2+jp}w_3{(w_4)}^j) \\
              & = &
              \del({(t_2t_1)}^{k_1+jn}t_2v_3{(v_4)}^j,{(t_2t_1)}^{k_2+jp}w_3{(w_4)}^j) \\
            \end{array}
            \]


          We now consider the following subcases:

          \begin{itemize}
          \item[2.3.1] $|v_2| > |w_2|$.
            As a consequence, $n>p$, and we can assume that $K$
            is big enough, so that $k_1-k_2+j(n-p)>0$.
            We get:
            \[
            \begin{array}{lllll}
              \del(V^{(j)},W^{(j)})
              & = &
              \del({(t_2t_1)}^{k_1-k_2+j(n-p)}t_2v_3{(v_4)}^j,w_3{(w_4)}^j)
              \\
              & = &
              \del({(t_2t_1)}^{k_1-k_2+j(n-p)}t_2v_3{(v_4)}^j,\alpha_1'b\alpha_3{(w_4)}^j)
              \\
              & = &
              \del({(t_2t_1)}^{k_1-k_2+j(n-p)}t_2v_3{(v_4)}^j,{(t_2t_1)}^{k_3}Xb\alpha_3{(w_4)}^j)
              \\
            \end{array}
            \]
            We can take $j$ such that $k_1-k_2+j(n-p)>k_3$, and
            therefore we finally have:
            \[
            \begin{array}{lllll}
              & & \del(V^{(j)},W^{(j)}) \\
              & = &
              \del({(t_2t_1)}^{k_1-k_2+j(n-p)-k_3}t_2v_3{(v_4)}^j,Xb\alpha_3{(w_4)}^j)
              \\
              & = &
              \del(XaY{(t_2t_1)}^{k_1-k_2+j(n-p)-k_3-1}t_2v_3{(v_4)}^{j},Xb\alpha_3{(w_4)}^j)
              \\
              & = &
              (aY{(t_2t_1)}^{k_1-k_2+j(n-p)-k_3-1}t_2v_3{(v_4)}^{j},b\alpha_3{(w_4)}^j)
            \end{array}
            \]
            Since $t_2t_1\neq\epsilon$, we get that the first
            component of the delay always increases in size when $j$ increases;

            \item[2.3.2] $|v_2|<|w_2|$. We can take $K$
              large enough such that this case never happens, i.e.
              ${(v_2)}^i$  and $w_3$ do not overlap.

            \item[2.3.3] $|v_2| = |w_2|$. Therefore $n = p$, and we
              have for all $j\geq i$:
              \[
              \begin{array}{lllll}
                \del(V^{(j)},W^{(j)}) = \del({(t_2t_1)}^{k_1}t_2v_3{(v_4)}^j,{(t_2t_1)}^{k_2}w_3{(w_4)}^j)
                \\
              \end{array}
              \]
              As case $2.3.1$, since by hypothesis there is an overlap between ${(v_2)}^i$
              and $w_3$, we have $k_1 > k_2 + k_3$, and we get:
              \[
              \begin{array}{lllll}
                \del(V^{(j)},W^{(j)}) & = & \del({(t_2t_1)}^{k_1-k_2}t_2v_3{(v_4)}^j,w_3{(w_4)}^j)
                \\
                & = & \del({(t_2t_1)}^{k_1-k_2}t_2v_3{(v_4)}^j,{(t_2t_1)}^{k_3}Xb\alpha_3{(w_4)}^j)
                \\
                & = & \del({(t_2t_1)}^{k_1-k_2-k_3}t_2v_3{(v_4)}^j,Xb\alpha_3{(w_4)}^j)
                \\
                & = & \del(XaY{(t_2t_1)}^{k_1-k_2-k_3-1}t_2v_3{(v_4)}^j,Xb\alpha_3{(w_4)}^j)
                \\
                & = & (aY{(t_2t_1)}^{k_1-k_2-k_3-1}t_2v_3{(v_4)}^j,b\alpha_3{(w_4)}^j)
                \\
              \end{array}
              \]
              Therefore if $v_4 \neq \epsilon$ and $w_4\neq\epsilon$,
              we are done as one of the two components of the delay
              will increase in size when $j$ increases. If $v_4 = w_4
              = \epsilon$ we can explicitly give the form of
              $\del(V^{(0)},W^{(0)})$ and $\del(V^{(1)},W^{(1)})$:
              \[
              \begin{array}{lllllll}
              \del(V^{(0)},W^{(0)}) & = & \del({(t_2t_1)}^{k_1}t_2v_3,
              {(t_2t_1)}^{k_2+k_3}Xb\alpha_3) \\
              & = &  \del({(t_2t_1)}^{k_1-k_2-k_3}t_2v_3,
              Xb\alpha_3) \\
              & = & \del({(t_2t_1)}^{k_1}t_2{(t_1t_2)}^{n}v_3,
              {(t_2t_1)}^{k_2+k_3+n}Xb\alpha_3) \\
              & = & \del(V^{(1)},W^{(1)}) \\
              \end{array}
              \]
              This is excluded by hypothesis, so this case is not possible.
          \end{itemize}

          \item[2.4] the other cases (the first difference occurs
            between ${(v_2)}^i$ and ${(w_4)}^i$, or between $v_3$ and
            $w_3$, or between $v_3$ and ${(w_4)}^i$, or between
            ${(v_4)}^i$ and ${(w_4)}^i$) are proved similarly as case 2.3 by
            decomposing the words as power of their primitive
            roots. For instance, if the first difference occurs
            between $v_3$ and $w_3$, then either $v_2 = w_2 =
            \epsilon$ and it is the same as case 2.1, or
            $v_2\neq\epsilon$ and $w_2=\epsilon$ but we can take $K$
            large enough so that this case is impossible, or
            $v_2\neq\epsilon$ and $w_2\neq\epsilon$. In this latter
            case we can take $K$ large enough so that the
            primitive roots of $v_2$ and $w_2$ are conjugate. We have
            again to distinguish several cases on the relative lengths
            of $v_2$ and $w_2$ (as for 2.3) but the proofs are
            similar. Similar techniques were already applied to
            prove that functionality is decidable for \vpts~\cite{DBLP:journals/corr/abs-1002-1443}.




%%         \item[2.7] there is $i\geq K$ such that $v_1(v_2)^i =
%%           \alpha_1a\alpha_2$ and $w_1(w_2)^iw_3(w_4)^i =
%%           \alpha_1b\alpha_3$, with $|\alpha_1|\geq |w_1(w_2)^iw_3|$
%%           (otherwise it is case 2.3).

%%         \item[2.8] there is $i\geq K$ such that $v_1(v_2)^iv_3 =
%%           \alpha_1a\alpha_2$ and $w_1(w_2)^iw_3 = \alpha_1b\alpha_3$
%%           with $|\alpha_1|\geq |v_1(v_2)^i$ and $|\alpha_1|\geq
%%           |w_1(w_2)^i|$.

%%         \item[2.9] there is $i\geq K$ such that $v_1(v_2)^iv_3 =
%%           \alpha_1a\alpha_2$ and
%%           $w_1(w_2)^iw_3(w_4)^i=\alpha_1b\alpha_2$ with
%%           $|\alpha_1|\geq |v_1(v_2)^i|$ and $|\alpha_1|\geq
%%           |w_1(w_2)^iw_3|$.

%%         \item[2.10] there is $i\geq K$ such that $v_1(v_2)^iv_3(v_4)^i
%%           = \alpha_1a\alpha_2$ and $w_1(w_2)^iw_3(w_4)^i =
%%           \alpha_1b\alpha_3$ with $|\alpha_1|\geq |v_1(v_2)^iv_3|$ and
%%           $|\alpha_1|\geq |w_1(w_2)^iw_3|$. Therefore $v_4\neq
%%           \epsilon$ and $w_4\neq\epsilon$.

%%           We have taken $K$ large
%%           enough so that $w_4^i$ and $v_4^i$ have a common subword of
%%           length at least $|w_4|+|v_4|$. Therefore there exist
%%           $t_1,t_2\in\Sigma^*$ and $n,p\geq 0$ such that $t_1t_2$ is
%%           primitive, $v_4 = (t_1t_2)^n$ and $w_4 = (t_2t_1)^p$.





      \end{itemize}


  \end{itemize}
            \end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:

